SATA-BENCH: Select All That Apply Benchmark for Multiple Choice Questions

Large language models (LLMs) are increasingly evaluated on single-answer multiple-choice tasks, yet many real-world problems require identifying all correct answers from a set of options. This capability remains underexplored. We introduce SATA-BENCH, the first dedicated benchmark for evaluating LLMs on Select All That Apply (SATA) questions across diverse domains, including reading comprehension, law, and biomedicine. Our evaluation of 27 open-source and proprietary models reveals a significant gap: even the strongest model achieves only 41.8% exact match, exposing LLMs' inability to reliably identify all correct answers. We find that this weakness stems from two core challenges: selection bias - models favor certain choices regardless of content, and count bias - models fail to predict the correct number of answers. To address these issues, we propose Choice Funnel, a decoding strategy that combines token debiasing with adaptive thresholding to guide models toward complete and accurate selections. Choice Funnel achieves up to 29% higher exact match than competitive baselines while reducing inference cost by over 64%. Our findings expose fundamental limitations in current LLMs and introduce a new framework for diagnosing and improving multi-answer reasoning. We release SATA-BENCH and Choice Funnel to promote LLM development for robust decision-making in realistic, multi-answer applications.

==> 0_Abstract/abstract_chomp.tex <==
\begin{abstract}
Current large language model (LLM) evaluations primarily focus on single-answer tasks, whereas many real-world applications require identifying multiple correct answers. This capability remains underexplored due to the lack of dedicated evaluation frameworks. We introduce \method, a benchmark for evaluating LLMs on Select All That Apply (SATA) questions spanning six domains, including reading comprehension, legal reasoning, and biomedicine. Our evaluation of 32 models demonstrates substantial limitations: the strongest model achieves only 75.3\% Jaccard Index and 41.8\% exact match accuracy. We identify the failure: speculation bias, models include incorrect answers when uncertain; In other words, models hallucinate a lot when answering completing \method. To address these limitations, we propose \textbf{Choice Funnel}, a decoding strategy that combines token debiasing with adaptive thresholding and abstention handling to guide models toward complete and accurate multi-answer selections. Choice funnel improves the accuracy of the exact match by up to 29\% while reducing the inference cost by more than 64\% compared to the existing approaches. We release \method and Choice Funnel to encourage the development of LLMs capable of robust decision-making in realistic multi-answer scenarios.
\end{abstract}

==> 1_Introduction/introduction_chomp.tex <==

\section{Introduction}  
\begin{wrapfigure}{r}{0.65\textwidth}  
\vspace{-1.8em}  
\includegraphics[height=5.2cm]{2_Benchmark/fig1_6.jpg}   
\small\caption{Representative example of an LLM failure on a SATA (Select All That Apply) question. Models often miss valid answers due to unselection, count, and speculation biases. Gemini speculates in this question while GPT-4o underselects. Other models may have unselection bias over C.}  
\label{fig:llm-struggle}  
\end{wrapfigure}  

Large Language Models (LLMs) have demonstrated remarkable capabilities across diverse natural language processing tasks, with multiple-choice question answering becoming a standard evaluation framework~\citep{pezeshkpour24,zheng2024largelanguagemodelsrobust}. However, current benchmarks assume a single correct answer per question, even though many applications require multiple valid responses, and because they rely on binary scoring that does not penalize speculation, they inadvertently encourage hallucination~\citep{kalai2025hallucinate}. Consider content moderation systems that must flag posts for several policy violations simultaneously, medical diagnosis tools that identify co-occurring conditions, or legal research platforms that classify documents under multiple relevant statutes. These scenarios represent Select All That Apply (SATA) tasks, where success depends not on choosing the single best option but on accurately identifying the complete set of correct answers. Despite their prevalence in real-world applications, SATA tasks remain underexplored in LLM evaluation, leaving a gap between benchmark performance and practical utility with direct implications for trustworthiness and safety. Existing evaluations overestimate model reliability by rewarding speculation, whereas SATA-specific metrics directly penalize speculative behavior and hallucination.  

To address this gap, we introduce \method, a comprehensive benchmark containing over 10,000 human-validated questions across six domains: reading comprehension, toxicity detection, news categorization, biomedicine, legal classification, and event analysis. Unlike existing multi-label classification datasets that often include dozens of possible labels and assume bag-of-words features, \method provides natural-language multiple-choice questions with 3–15 options and 2–10 correct answers, together with metrics that evaluate option-order effects, abstention behavior, and other phenomena unique to LLMs. 

Our evaluation of 32 state-of-the-art models (including both proprietary LLMs and open-source alternatives) reveals substantial limitations in multi-answer reasoning. Even the best-performing model achieves only 41.8\% exact match accuracy, missing the full correct set in nearly 60\% of questions. Figure~\ref{fig:llm-struggle} illustrates a representative failure where models correctly identify some valid answers but systematically avoid others. We identify three speculation bias\footnote{We use the term bias to highlight systematic tendencies in prediction (See Appendix~\ref{sec:bias_definition} for mathematical definitions), not socioeconomic or demographic bias } underlying these failures: \textit{speculation bias}, where models include incorrect options when uncertain rather than abstaining~\citep{kalai2025hallucinate}. To mitigate these issues, we propose \textit{Choice Funnel}, a decoding algorithm that combines token debiasing, adaptive thresholding, and abstention handling. Beyond evaluation, \method serves as both a benchmark and a diagnostic platform, revealing systematic failure modes and enabling algorithmic advances such as Choice Funnel.  

\textbf{Our Contributions.} The primary contributions of this paper are:
\vspace{-0.1in}
\begin{enumerate}[leftmargin=*]
\item \textit{\method Data Curation}: We curate a high-quality, diverse benchmark dataset explicitly designed to challenge LLMs on multi-answer tasks. \method contains more than 10K human-validated questions with multiple domains, varying difficulty levels, multiple correct answers, and carefully constructed distractors. In addition, we provide readability, confusion, and similarity analyses to ensure clarity, diversity, and task complexity across six domains. Unlike other datasets,  \method penalize any speculation and hallucination. 

\item \textit{Comprehensive Evaluation}: We conduct the largest-to-date evaluation of 32 proprietary and open-source LLMs on SATA questions, revealing that even the strongest models achieve only 41.8\% exact match accuracy and 75.3\% Jaccard Index.  

\item \textit{Bias Diagnosis}: We identify and formalize \textit{speculation} biases as obstacles to solving SATA questions, and introduce multiple metrics to evaluate speculation biases. 

\item \textit{Choice Funnel Algorithm}: We introduce a decoding strategy that jointly mitigates these biases through token debiasing, adaptive thresholding, and abstention handling, improving exact match accuracy by up to 29 percentage points while reducing inference cost by 64\%.  
\end{enumerate}
\vspace{-0.1in}

% could still work in:
% Existing benchmarks such as MMLU-Pro, GPQA, and BBH rely on \textit{binary grading} (i.e., models receive credit only if the exact answer set is predicted) and provide no recognition for abstentions, which further incentivizes hallucination \citep{kalai2025hallucinate}. 






%Large Language Models (LLMs) have demonstrated remarkable success across a variety of natural language processing tasks, with multiple-choice question (MCQ) answering emerging as a prominent evaluation setting \citep{pezeshkpour24,zheng2024largelanguagemodelsrobust}. However, most existing benchmarks and training pipelines focus on questions with a \textit{single} correct answer evaluated solely by exact accuracy. Recent works~\citep{kalai2025hallucinate} have shown that these benchmarks encourage speculation and overstate model reliability. As a result, they fail to reflect real-world tasks that often require identifying \textit{multiple} correct answers.


% could still work in:
% Existing benchmarks such as MMLU-Pro, GPQA, and BBH rely on \textit{binary grading} (i.e., models receive credit only if the exact answer set is predicted) and provide no recognition for abstentions, which further incentivizes hallucination \citep{kalai2025hallucinate}. 






%Large Language Models (LLMs) have demonstrated remarkable success across a variety of natural language processing tasks, with multiple-choice question (MCQ) answering emerging as a prominent evaluation setting \citep{pezeshkpour24,zheng2024largelanguagemodelsrobust}. However, most existing benchmarks and training pipelines focus on questions with a \textit{single} correct answer evaluated solely by exact accuracy. Recent works~\citep{kalai2025hallucinate} have shown that these benchmarks encourage speculation and overstate model reliability. As a result, they fail to reflect real-world tasks that often require identifying \textit{multiple} correct answers.

%Many practical applications naturally require multiple correct answers. For instance, a social media moderator may need to tag a post for several types of toxic content—such as threats, hate speech, or offensive language. Similarly, biomedical researchers annotating papers or journalists extracting facts from news articles must often identify multiple relevant subdomains simultaneously. These are instances of \textbf{Select All That Apply (SATA)} questions, where more than four options are presented and several may be correct. Unfortunately, even advanced LLMs struggle in such scenarios: while they achieve high precision on individual options, they consistently fail to recover the full set of answers, as illustrated in Figure~\ref{fig:llm struggle}.

%We identify three key sources of this failure. First, \textit{unselection bias}: models systematically disfavor certain labels regardless of correctness. Second, \textit{count bias}: models underpredict the number of valid answers, omitting correct ones. Third, \textit{speculation bias}: when uncertain, models overgenerate by selecting spurious answers. Together, these biases explain why even the strongest LLMs score below $50\%$ exact match on SATA tasks despite strong single-answer performance.

% To address this challenge, we propose \textbf{Choice Funnel}, a decoding algorithm specifically designed for multi-answer reasoning. Choice Funnel integrates (i) \textit{token debiasing} to counter skewed option probabilities, (ii) \textit{adaptive thresholding} to mitigate under-selection, and (iii) an abstention mechanism (\textit{None of the Above}) to reduce speculation. This lightweight procedure improves exact match accuracy by up to 29 percentage points and cuts inference cost by 64\% compared to naive option-by-option prompting. Studying these biases also requires the right evaluation setting. Existing benchmarks such as MMLU-Pro, GPQA, and BBH rely on \textit{binary grading} (i.e., models receive credit only if the exact answer set is predicted) and provide no recognition for abstentions, which further incentivizes hallucination \citep{kalai2025hallucinate}. To enable principled evaluation, we introduce \method, a human-validated multi-domain benchmark of over 10K multi-answer questions. Unlike prior benchmarks, \method employs metrics such as the Jaccard Index that explicitly penalize speculation.  



==> 3_Experiments/choice.tex <==
\section{The Choice Funnel Algorithm}
\label{sec:choicefunnel}

\subsection{Design Goals}
Section~\ref{sec:challenge} showed that LLM errors on SATA arise from two systematic effects:
(i) \emph{selection skew/avoidance} over option IDs and (ii) pervasive \emph{count underestimation}.
A practical decoding algorithm should therefore (a) counter option-ID priors (\emph{debias}),
(b) adaptively decide \emph{how many} to select, and (c) allow \emph{abstention} when appropriate,
all while keeping inference cost low.

\subsection{Debias--then--Select with Abstention}
Let $\mathcal{O}=\{o_1,\dots,o_K\}$ be the current option set and let $\pi_\theta$ denote the LLM.
From the first-token distribution over option identifiers, we compute a \emph{debiased} score
$\tilde p(o) = \mathrm{DebiasingFunction}\!\left(\pi_\theta(\cdot \mid \mathbf{P})\right)[o]$,
where $\mathbf{P}=\mathrm{MakeSATAPrompt}(\mathcal{T},\mathcal{O})$ is the prompt for task $\mathcal{T}$.
In practice, we instantiate \texttt{DebiasingFunction} with a label-free prior-correction such as PriDe
\citep{zheng2024largelanguagemodelsrobust} (adapted to SATA; see Appendix).

We iteratively select the highest-scoring option and remove it from $\mathcal{O}$.
To enable uncertainty-aware stopping, we include a special option \texttt{NOTA} (\emph{None of the above}),
motivated by survey methodology that endorses explicit IDK/NOTA responses
\citep{schumanpresser1996,Eckman2024}.
Following our ablations, we introduce \texttt{NOTA} after at least one selection
(to avoid premature stopping on initialization), and we stop when either \texttt{NOTA} is selected
or the remaining top debiased score falls below a confidence floor $\tau$.


\begin{algorithm}[H]
\fontsize{8.5}{8.5}\selectfont
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Choice Funnel}
\Input{LLM $\pi_{\theta}$, SATA problem $\mathcal{T}$, option set $\mathcal{O}$, $NOTA$ stop option, $\tau$ confidence threshold}
\Output{Selected set $\mathcal{R}$}
$\mathcal{R} \gets \emptyset$; $\mathcal{O}_{work}\gets\mathcal{O}$ \\
\While{$\mathcal{O}_{work} \neq \emptyset$}{
    {\textcolor{gray}{\# Build prompt over current options}}\\
    $\mathbf{P} \gets \text{MakeSATAPrompt}(\mathcal{T}, \mathcal{O}_{work})$\\
    {\textcolor{gray}{\# Debiased first-token probabilities}}\\
    $\tilde p \gets \text{DebiasingFunction}(\pi_{\theta}(\cdot \mid \mathbf{P}))$\\
    {\textcolor{gray}{\# Take top option and score}}\\
    $o \gets \arg\max_{x \in \mathcal{O}_{work}} \tilde p(x)$; \quad $m \gets \tilde p(o)$\\
    {\textcolor{gray}{\# Stop if low confidence or abstention}}\\
    \If{$m < \tau$}{\textbf{break}}
    \If{$o = \text{NOTA}$}{\textbf{break}}
    {\textcolor{gray}{\# Accept and continue}}\\
    $\mathcal{R} \gets \mathcal{R} \cup \{o\}$\\
    \If{$\text{length}(\mathcal{R}) = 1$ \textbf{and} $NOTA \notin \mathcal{O}_{work}$}{
        $\mathcal{O}_{work} \gets \mathcal{O}_{work} \cup \{\text{NOTA}\}$
    }
    $\mathcal{O}_{work} \gets \mathcal{O}_{work} \setminus \{o\}$\\
}
\end{algorithm}


\paragraph{Discussion.}
(i) \textbf{Plug-and-play debiasers.} Any single-answer MCQ debiaser that estimates option-ID priors
(e.g., via random permutations) can be slotted into \texttt{DebiasingFunction}; we adopt PriDe
\citep{zheng2024largelanguagemodelsrobust} for its label-free, efficient implementation.
(ii) \textbf{Stopping rules.} \texttt{NOTA} implements abstention; the confidence floor $\tau$
prevents the common failure where long tails of near-zero scores trigger over-selection or noisy picks.
(iii) \textbf{Scheduling \texttt{NOTA}.} Adding \texttt{NOTA} only after the first selection improved stability in our ablations
(Appendix).

\subsection{Theoretical Intuition and Properties}
We provide lightweight analysis to clarify why Choice Funnel reduces both selection and count bias.

\paragraph{Selection skew reduction.}
Assume a simple additive prior model for the (logit) score of option $o$:
$s(o)=q(o)+b(o)$, where $q(o)$ encodes task evidence and $b(o)$ is an option-ID prior (format/position bias).
Let $\tilde s(o)=s(o)-\hat b(o)$ be the debiased score using an estimator $\hat b(o)$ obtained by content permutations.
Under $\mathbb{E}[\hat b(o)] = b(o)$ and bounded estimation error, the between-option variance of debiased selection
probabilities decreases, reducing selection skew as measured by RStd/RSD
\citep{croce2020robustbench,reif2024calibration,zheng2024largelanguagemodelsrobust}.
\emph{Proof sketch:} subtracting a consistent prior removes a common offset component in $s(\cdot)$,
shrinking dispersion and flattening spurious preferences.

\paragraph{Count underestimation correction.}
Let $m_t=\max_{o\in\mathcal{O}_t}\tilde p_t(o)$ be the top debiased score at iteration $t$.
If the true set size is $C^\star$ and $m_t$ is stochastically non-decreasing for true positives
as $\mathcal{O}_t$ prunes false options, then stopping when $m_t<\tau$ induces an \emph{adaptive} estimate of
$|\hat S|$ that increases with evidence strength, mitigating the global under-selection bias observed in Sec.~\ref{sec:challenge}.

\paragraph{Inference cost.}
\begin{proposition}
Let $T$ be the number of iterations until stopping (either by \texttt{NOTA} or $m_t<\tau$). Choice Funnel requires
$T$ forward passes and outputs $|\mathcal{R}|=T'$ selections with $T'\le T\le T'+1$.
In particular, if the procedure halts immediately after rejecting the $(T'\!+\!1)$-st candidate (by $m_t<\tau$ or \texttt{NOTA}),
then $T = T'\!+\!1$. Compared to option-by-option yes/no prompting with cost $\Theta(K)$,
Choice Funnel scales with the (typically small) number of selected answers.
\end{proposition}

\noindent
\emph{Discussion.} Empirically, we observe $T' \approx C^\star$ when selection bias is corrected and $\tau$ is reasonably calibrated,
so the number of forward passes scales roughly with the number of \emph{correct} labels rather than total options $K$,
matching the efficiency gains in our experiments.

\subsection{Implementation Choices}
We instantiate \texttt{DebiasingFunction} with an adaptation of PriDe
\citep{zheng2024largelanguagemodelsrobust}, estimating option-ID priors via random permutations of option contents on a small holdout,
then subtracting these priors at inference. The confidence floor $\tau$ is fixed across models for simplicity;
ablation of $\tau$ and the \texttt{NOTA} schedule is reported in the Appendix.
Appendix also details prompts and the minor modifications needed to apply PriDe in the SATA setting.


==> 3_Experiments/experiments_chomp.tex <==
\section{Experiments}\label{sec:experiments}
%\vspace{-0.1in}
This section presents the experiments conducted to assess the capabilities of LLMs on SATA questions on evaluation set. Our benchmark covers 18 proprietary and 14 open-source models (see Table~\ref{tab:model_cards} for details). Because the benchmark spans diverse domains, we adopt a zero-shot evaluation protocol. The system prompt specifies that each question has at least two correct answers, and we instruct the LLM to output the results in JSONL format~\citep{Intelligence2024, zhou2023instructionfollowingevaluationlargelanguage}. Furthermore, we employ a CoT prompting strategy following~\citep{openai2024gpt4technicalreport}. We then extract answers from the JSONL output using exact and fuzzy match. For cases where JSONL extraction fails (fewer than 3\%), we use Claude 3 Haiku and human labelers to recover the correct options. However, for smaller models, the JSONL extraction fails in more than 5\% of the cases, making this method less reliable. In these cases, following~\citep{hendrycks2021measuringmassivemultitasklanguage}, we omit CoT and instead rank options using the probability of the first output token. To calibrate thresholds, we hold out 100 randomly sampled instances from the benchmark and tune each model for the optimal Jaccard Index~\citep{bogatinovski2022comprehensive}. We then select all options with probabilities above this threshold. This probability-based method applies only to models with accessible token likelihoods. Finally, we also evaluate the performance of non-expert humans on the benchmark (Appendix~\ref{appedix:human_eval}).  

%:  Claude 3.5 Haiku, Claude 3.5 Sonnet V1, Claude 3 Opus, Claude 3 Haiku, Claude 3 Sonnet, Claude 3.7, Claude 3.7 with thinking~\citep{claude2024}, Gemini 2 Flash, Gemini 2.5 Flash Thinking~\citep{team2023gemini}, GPT4o, O3, GPT 4.1, GPT 4.1 mini~\citep{openai2024gpt4technicalreport}, Grok 3 think, Nova Pro, Nova Micro, Nova Lite~\citep{Intelligence2024}, DeepSeek R1,  DeepSeek R1 Distill Llama 8B~\citep{deepseekai2025deepseekr1}, Qwen Plus, Qwen2.5 14B~\citep{qwen2025qwen25technicalreport}, Mistral Large V2~\citep{jiang2023mistral}, Ministral 8B~\citep{ministraux2024}, Phi 3 7B~\citep{abdin2024phi}, Phi 4 mini reasoning~\citep{abdin2025phi4reasoning}, Bloomz 7B~\citep{muennighoff2022crosslingual}, Llama 3.1 70B, Llama 3.2 90B, Llama 3.1 8B, and Llama 3.1 405B~\citep{touvron2023llama}.

% \textbf{Metrics.} We evaluate models using metrics across three categories: performance, selection bias, and count bias (details in Appendix~\ref{app:metrics}). Performance is measured using Exact Match (EM), Jaccard Index (JI), Mean Average Precision (Precision), and False Positive Rate (FPR). Selection bias includes RStd~\citep{zheng2024largelanguagemodelsrobust} and RSD~\citep{croce2020robustbench, reif2024calibration}. We also introduce Selection Probability Divergence (SPD) to quantify unselection bias, a form of selection bias where models consistently avoid certain options. Count bias is assessed using the mean count difference (CtDif), mean absolute count difference (CtDifAbs), and count accuracy (CtAcc).

\begin{table*}[h!]
\centering
\vspace{0.1in}

\caption{Performance comparison of 32 different LLMs across various metrics on \method. We highlight the best (\textbf{bold}) and second-best (\underline{underline}) values.
Columns labeled [(\(\uparrow\))] indicate higher-is-better; columns labeled [(\(\downarrow\))] indicate lower-is-better. Models with explicit reasoning capabilities are highlighted in \textit{italic}. All numeric values are rounded to two decimal places. We retrieve exact labels for models evaluated using Inference-Based Retrieval + CoT prompting. For models evaluated under Probability-Based Retrieval, we select labels based on token probability thresholds.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}  
\toprule
& \multicolumn{4}{c}{\textbf{Performance}} 
& \multicolumn{3}{c}{\textbf{Selection Bias}}
& \multicolumn{3}{c}{\textbf{Count Bias}} 
\\
\cmidrule(lr){2-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
\textbf{Model Name} &
\textbf{JI}\(\uparrow\) &
\textbf{FPR}\(\downarrow\) &
\textbf{EM}\(\uparrow\) &
\textbf{Precision}\(\uparrow\) &
\textbf{SPD}\(\downarrow\) &
\textbf{RStd}\(\downarrow\) &
\textbf{RSD}\(\downarrow\) &
\textbf{CtDif} &
\textbf{CtDifAbs}\(\downarrow\) &
\textbf{CtAcc}\(\uparrow\) \\
\midrule
\multicolumn{11}{c}{\textbf{Inference Based Retrieval + CoT}}\\
\hdashline\\[-1.5ex]
\textit{O3}                          & 73.91 & 31.58 & \textbf{41.77} & 87.50 & 0.38 & 6.79 & \underline{0.06} & -0.39 & 0.94 & 46.12 \\
GPT 4.1                               & \textbf{75.23} & 40.37 & \underline{40.49} & 85.52 & \underline{0.13} & \underline{5.98} & \underline{0.06} & -0.04 & 0.85 & 45.52 \\
\textit{GPT-OSS 120B}                & 74.28 & 37.53 & 40.29 & 86.28 & 0.19 & 6.31 & 0.07 & -0.16 & 0.84 & \underline{47.57} \\
\textit{Grok 3 Think}                & \underline{74.40} & 43.10 & 39.71 & 83.93 & 0.30 & 6.26 & 0.07 &  0.06 & 0.93 & 44.24 \\
GPT 4                                 & 74.11 & 38.42 & 39.47 & 85.90 & 0.21 & 6.63 & \underline{0.06} & -0.20 & \textbf{0.82} & 46.61 \\
\textit{Claude 3.7 Think}            & 70.96 & 35.16 & 37.92 & 85.03 & 0.46 & 18.77 & 0.34 & -0.32 & 0.87 & 44.48 \\
Claude 3.7                           & 70.98 & 33.10 & 37.82 & 85.35 & 0.49 & 6.59 & 0.25 & -0.43 & 0.93 & 43.58 \\
Claude 3 Sonnet                      & 70.72 & 38.81 & 36.49 & 84.58 & 0.36 & 7.37 & 0.07 & -0.35 & \underline{0.83} & \textbf{48.00} \\
\textit{Geimini 2.5 Think}           & 72.58 & 42.16 & 36.46 & 84.58 & \textbf{0.12} & \textbf{4.76} & \underline{0.06} &  -0.01 & 0.88 & 43.76 \\
Claude 3.5 Haiku                     & 71.12 & 50.01 & 35.89 & 80.26 & 0.33 & 7.31 & 0.35 &  0.18 & 1.01 & 42.61 \\
Claude 3 Haiku                       & 70.63 & 40.84 & 35.64 & 83.59 & 0.42 & 6.24 & 0.07 & -0.22 & 0.85 & 47.15 \\
Claude 3 Opus                        & 70.15 & 34.17 & 35.59 & 86.97 & 0.62 & 8.26 & 0.07 & -0.52 & 0.93 & 44.36 \\
Gemini 2 Flash                       & 70.71 & 40.79 & 34.60 & 85.01 & 0.17 & 6.14 & \underline{0.06} & -0.23 & 0.91 & 39.94 \\
GPT 4.1 mini                         & 69.90 & 37.31 & 33.46 & 86.05 & 0.30 & 6.69 & \underline{0.06} & -0.39 & 0.97 & 38.61 \\
Nova Pro                             & 68.92 & 31.64 & 32.95 & 87.37 & 0.52 & 7.92 & 0.07 & -0.55 & 1.01 & 39.27 \\
Claude 3.5 Sonnet                    & 67.15 & 34.25 & 32.22 & 87.57 & 0.43 & 8.41 & 0.09 & -0.46 & 1.06 & 38.55 \\
Llama 3.1 405B                       & 67.18 & 35.06 & 30.17 & 86.24 & 0.33 & 6.90 & 0.45 & -0.39 & 1.02 & 36.30 \\
Nova Lite                            & 63.75 & 39.88 & 29.11 & 82.51 & 0.52 & 9.12 & 0.45 & -0.51 & 1.17 & 37.39 \\
\textit{Deepseek R1}                 & 64.49 & 34.89 & 28.17 & 84.62 & 0.94 & 17.44 & \textbf{0.03} & -0.57 & 1.13 & 33.52 \\
\textit{GPT-OSS 20B}                 & 60.73 & 40.90 & 27.35 & 80.90 & 0.77 & 11.05 & 0.10 & -0.53 & 1.45 & 31.80 \\
Mistral Large V2                     & 57.16 & 27.23 & 22.83 & \textbf{88.20} & 1.33 & 10.89 & 0.12 & -1.10 & 1.47 & 27.27 \\
Qwen Plus                            & 55.74 & 24.03 & 21.12 & 88.54 & 2.24 & 10.72 & 0.11 & -1.18 & 1.43 & 24.85 \\
Nova Micro                           & 55.77 & 29.28 & 18.37 & 86.06 & 1.84 & 11.10 & 0.27 & -1.09 & 1.41 & 24.30 \\
Llama 3.2 90B                        & 55.78 & \textbf{23.81} & 18.30 & \textbf{89.56} & 1.84 & 11.10 & 0.27 & -1.09 & 1.41 & 24.30 \\
Llama 3.1 70B                        & 55.59 & \underline{23.92} & 17.94 & \textbf{89.56} & 1.81 & 10.06 & 0.10 & -1.12 & 1.48 & 22.12 \\
Non-expert Human                     & 45.02 & -- & 17.93 & 60.62 & 1.46 & 15.32 & 1.46 & -0.6 & 1.44 & 34.12 \\
\midrule
\multicolumn{11}{c}{\textbf{Probability Based Retrieval}}\\
\hdashline\\[-1.5ex]
Mistral 8B                           & \textbf{46.63} & 32.21 & \textbf{14.73} & \underline{81.46} & \textbf{11.42} & 19.47 & 1.27 & -1.35 & 1.95 & \underline{21.01} \\
Llama3 8B                            & \underline{43.64} & 30.06 & \underline{13.82} & 80.30 & \underline{12.09} & \underline{17.85} & \underline{1.09} & -1.59 & 1.88 & \textbf{22.00} \\
Bloomz 7B                            & 41.15 & 57.76 & 11.27 & 66.09 & 20.62 & 29.00 & 1.51 & \textbf{-0.87} & \textbf{1.71} & 20.09 \\
\textit{DeepSeek R1 Distill 8B}      & 40.02 & 45.33 & 8.85 & 72.20 & 13.38 & 21.62 & 1.14 & \underline{-1.29} & \underline{1.75} & 20.42 \\
Qwen2.5 14B                          & 37.58 & \textbf{17.27} & 6.30 & 87.84 & 21.01 & 18.02 & \textbf{1.06} & -2.24 & 2.26 & 11.93 \\
Phi3 7B                              & 34.57 & \underline{17.64} & 2.97 & \textbf{87.25} & 23.22 & 18.57 & \underline{1.22} & -2.33 & 2.35 & 7.22 \\
\textit{Phi4-mini-reasoning}         & 29.69 & 26.73 & 2.12 & 77.98 & 21.62 & \textbf{13.90} & 1.59 & -2.37 & 2.39 & 7.35 \\
\bottomrule
\end{tabular} }
\label{tbl:model_results_no_f1}
\end{table*}
\vspace{-0.05in}
\subsection{Evaluation Metrics} \label{sec:metrics}
\vspace{-0.05in}
Evaluation of SATA question responses requires metrics that capture partial correctness , penalize inappropriate selections, and identify bias. We organize our evaluation into three categories: performance metrics that measure correctness and speculation, selection bias metrics that quantify positional preferences, and count bias metrics that assess quantity prediction accuracy. Detailed explanations for all metrics appear in Appendix~\ref{app:metrics}.
\vspace{-0.1in}
\textbf{Performance and Speculation Bias Metrics.} We employ four metrics to assess answer correctness~\citep{tarekegn2024deep}. \textit{Jaccard Index (JI)} measures the intersection-over-union between predicted and gold labels, providing credit for partial matches. A low JI also reflects limited overlap between predicted and gold labels, indicating speculation bias. \textit{False Positive Rate (FPR)} measures the proportion of questions where models select any incorrect option, directly quantifying speculation bias. \textit{Exact Match (EM)} requires the predicted set to exactly match the gold set, representing the most stringent evaluation criterion. \textit{Mean Average Precision (Precision)} evaluates the fraction of selected answers that are correct, which also gives credits to partial correctness. 

% \textbf{(Un)selection Bias Metrics.} To characterize positional preferences, we measure models' tendencies to favor or avoid specific option positions. We use \textit{RStd}~\citep{zheng2024largelanguagemodelsrobust} and \textit{RSD}~\citep{croce2020robustbench,reif2024calibration} to quantify selection bias toward particular option IDs. Additionally, we introduce \textit{Selection Probability Divergence (SPD)} to measure unselection bias—the systematic tendency to avoid certain options regardless of content (detailed in Appendix~\ref{app:unselection}).

% \vspace{-0.01in}
% \textbf{Count Bias Metrics.} Models often select fewer options than warranted, necessitating specialized metrics for quantity assessment. We measure: (i) mean signed difference between selected and correct counts (\textit{CtDif}), where negative values indicate under-selection; (ii) mean absolute difference (\textit{CtDifAbs}) to quantify magnitude regardless of direction; and (iii) percentage of cases with exact count matches (\textit{CtAcc}) to assess quantity prediction accuracy. 
% \vspace{-0.1in}


% \subsection{Evaluation Metrics} 
% We report Jaccard Index (JI), Exact Match (EM), mean Average Precision (Precision), and False Positive Rate (FPR)~\citep{tarekegn2024deep}. JI measures the intersection-over-union between predicted and gold labels. EM requires the predicted set to exactly match the gold set. Precision and JI provide graded (non-binary) credit, and all three metrics penalize over-selection. FPR measures the share of questions where the model selects any label outside the gold set (i.e., explicit speculation). To characterize positional preferences, we measure \textit{selection bias} (a model’s tendency to favor specific option IDs) using RStd~\citep{zheng2024largelanguagemodelsrobust} and RSD~\citep{croce2020robustbench,reif2024calibration}; we also observe \textbf{unselection bias}, where models avoid choosing certain options, and introduce \textit{Selection Probability Divergence} (SPD) to quantify it (Appendix~\ref{app:unselection}). Finally, models tend to select fewer options than warranted (\textit{count bias}); we assess its severity via (i) the mean signed difference between selected and correct counts (CtDif), (ii) the mean absolute difference (CtDifAbs), and (iii) the percentage of cases with an exact count match (CtAcc). Detailed explanations of all metrics are provided in Appendix~\ref{app:metrics}.
% \textbf{Performance.} We report Exact Match (EM), Jaccard Index (JI), mean Average Precision (Precision), and False Positive Rate (FPR)~\citep{tarekegn2024deep}. JI is the intersection-over-union between the predicted and gold label sets; EM requires an exact set match; JI and Precision provide graded (non-binary) credit, and all three penalize over-selection. FPR measures the share of questions where the model selects any label outside the gold set (i.e., explicit speculation). (details in Appendix \ref{app:metrics})

% \textbf{(Un)selection Bias.} Selection bias is a model's preference for selecting specific option IDs as answers, and is measured by RStd~\citep{zheng2024largelanguagemodelsrobust} and RSD~\citep{croce2020robustbench, reif2024calibration}. We also observe that some models prefer to avoid selecting certain options, which we call \textbf{unselection bias}. We introduce a metric called \textit{Selection Probability Divergence} (SPD) to measure this type of bias. Appendix~\ref{app:unselection} give more details on this issue and the design of SPD. 

% \textbf{Count Bias.} We observe that models tend to select fewer number of options compared to the ground truth. We refer to this as \textit{Count Bias}. To evaluate the severity of this type of bias, we measure the following: (i) Mean difference between the number of selected options minus correct options (CtDif), (ii) Mean absolute difference between the number of selected options minus correct options (CtDifAbs), and (iii) Percentage of cases where the model selects exactly the correct number of options (CtAcc).



% @shixian: can you provide more details about how you retrieve probability?
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table*}[ht]
% \centering
% \small
% \begin{tabular}{lccccccccccc}
% \hline
% \textbf{Model Name} & 
% \textbf{EM} & 
% \textbf{HA} & 
% \textbf{F1} &
% \textbf{Recall} &
% \textbf{Precision} &
% \textbf{SPD} & 
% \textbf{ckld} & 
% \textbf{rstd} & 
% \textbf{DiffLen} & 
% \textbf{StdLen} & 
% \textbf{Abslen} \\
% \hline
% GPT4o               & 38.56 & 73.47 & 84.02 & 82.60 & 85.49 & 0.22 & 0.03 & 6.64 & -0.21 & 1.31 & 0.84 \\
% Claude 3 Sonnet     & 35.93 & 70.25 & 81.21 & 78.37 & 84.28 & 0.37 & 0.07 & 7.43 & -0.36 & 1.32 & 0.84 \\
% Claude 3 Haiku      & 35.21 & 70.19 & 81.51 & 79.77 & 83.33 & 0.42 & 0.06 & 6.29 & -0.23 & 1.39 & 0.86 \\
% Claude 3.5 Haiku    & 35.05 & 70.49 & 82.08 & 84.45 & 79.86 & 0.32 & 0.08 & 7.09 &  0.17 & 1.59 & 1.02 \\
% Claude 3 Opus       & 34.79 & 69.58 & 81.34 & 76.71 & 86.58 & 0.63 & 0.11 & 8.33 & -0.54 & 1.44 & 0.94 \\
% Nova Pro            & 34.71 & 69.51 & 81.14 & 75.38 & 86.94 & 0.55 & 0.05 & 8.15 & -0.56 & 1.47 & 1.02 \\
% Geinini 2.0 Flash   & 33.84 & 70.19 & 82.06 & 79.52 & 84.69 & 0.17 & 0.02 & 6.24 & -0.24 & 1.34 & 0.92 \\
% Claude 3.5 Sonnet V1 
%                     & 31.67 & 66.64 & 80.50 & 74.80 & 87.16 & 0.44 & 0.08 & 8.44 & -0.47 & 1.56 & 1.07 \\
% Llama 3.1 405B      & 29.62 & 66.66 & 79.99 & 74.89 & 85.85 & 0.35 & 0.45 & 6.97 & -0.40 & 1.47 & 1.03 \\
% Nova Lite           & 28.86 & 63.42 & 80.74 & 72.08 & 82.32 & 0.52 & 0.07 & 7.98 & -0.52 & 1.84 & 1.18 \\
% Mistral Large V2    & 22.46 & 56.79 & 72.30 & 62.25 & 87.97 & 1.39 & 0.06 & 10.26 & -1.11 & 1.85 & 1.48 \\
% Llama 3.2 90B       & 19.57 & 58.67 & 74.59 & 60.82 & 89.27 & 1.23 & 0.09 & 9.30 & -1.13 & 1.75 & 1.49 \\
% Nova Micro          & 18.24 & 55.54 & 71.21 & 60.79 & 85.96 & 1.86 & 0.27 & 11.12 & -1.10 & 1.67 & 1.42 \\
% Llama 3.1 70B       & 17.57 & 55.18 & 71.96 & 60.30 & 89.24 & 1.64 & 0.06 & 10.22 & -1.14 & 1.74 & 1.50 \\
% DeepSeek V3         &  9.87 & 42.29 & 59.63 & 44.58 & 90.04 & 6.09 & 0.01 & 17.29 & -1.98 & 2.07 & 2.14 \\
% \hline
% \end{tabular}
% \caption{Results of Evaulation of 24 Models on SATA-Bench. First 5 columns multiplied by 100, and all numeric values shown to 2 decimal places. Models sorted by EM.} \label{tbl:model_results}
% \end{table*}
%For example, GPT4o almost double the performance of Llama 3.2 90B in EA. 
% \textbf{LLMs prefer to making sure all selected questions are correct (precision) instead of selecting all correct answers (high exact matching) } 

% \vspace{10pt}
\subsection{Key Observations} \label{sec:key_observations}
\textbf{\method is challenging and different.} 13 models achieve a JI above $70\%$, but none surpass $42\%$ EM. This shows that while models often identify some correct answers, they fail to consistently recover the full set. 

Proprietary models generally achieve higher JI and Precision than open-source ones. Unlike other benchmarks, no single model dominates across all metrics. Notably, larger and more recent models do not always perform better. For instance, Claude 3 Sonnet outperforms Claude 3.5 Sonnet and Claude 3 Opus in exact match, though within the Claude family, larger models consistently have higher precision (e.g., Claude 3 Opus has the highest precision among the Claude 3 variants). According to~\citep{claude2024, deepseekai2024deepseekv3technicalreport}, these results contrast with performance on single-choice MCQ benchmarks such as MMLU~\citep{hendrycks2021measuringmassivemultitasklanguage} and ARC~\citep{clark2018thinksolvedquestionanswering}, where larger or newer models typically show clear gains. Large reasoning models (LRMs) are slightly better than their non-reasoning counterparts in JI but failed to reduce selection and count bias. We provide a case study in Appendix~\ref{reason_case} to investigate LRM's behavior. 

%It may be that newer and larger model cares more about precision and thus underpredict the number of correct choices. This is also why Claude 3.5 Sonnet V1 has the highest count difference across all Claude model family. 
%The lowest average count difference between predicted number of choices and actual number of choice is 0.84.   

%linear regression on number of actual count (X) on number of predicted count (Y). Across all model family, the highest coefficients is Llama 3.1 405B, which 0.62. This means that per correct count increase, the number of predicted count only increases 0.62. This lead to extreme low exact matching rate when the number of correct count is above 7. 


% \textbf{Models choose too few answers.} Nearly all LLMs tend to select fewer answers than required. For example, Llama 3.1 70B selects, on average, one fewer option per question than the correct number. Accordingly, it achieves the highest precision but the lowest Jaccard Index (JI). The tendency to under-select increases as the number of correct answers grows (Figure~\ref{fig:plot2}), which in turn depresses JI for questions with many correct choices (Figure~\ref{fig:plot1}). Even the best model achieves a CtAcc of only 48\%, predicting the correct number of answers in fewer than half of the questions. We hypothesize that this behavior stems from models being primarily trained and evaluated on benchmarks with single correct answers, making them poorly suited for SATA tasks. A t-test confirms this under-selection: the mean of CtDif is significantly below 0, with $p = 1.70 \times 10^{-6}$.

\textbf{Models speculate a lot.} LLMs also over-select, consistently choosing incorrect options, with all models exceeding a 20\% FPR. More than 70\% of the models predict at least one incorrect choice more often than they produce exact matches, underscoring their speculating behavior. Interestingly, stronger-performing models tend to speculate more: hallucination rate and exact match are positively correlated ($r = 0.61$, $p = 8 \times 10^{-4}$). This dual trend suggests that as models improve in identifying correct answers, they also become more prone to speculation, highlighting the difficulty of disentangling genuine knowledge from overconfidence in LLM predictions. This means that current LLMs hallucinates a lot and recent LLM hallucinates even more. 

% 1. All LLM has over 20 haullucination rate
% 2. More than 70\% models have higher hallucination rate than exact match rate. This shows that LLMs are highly incapable of solving questions with multiple correct answers.
% 3. Better performed model tends to have high hallucination rate. Suprisingly, the hallucination rate is highly correlated with exact match rate. This shows that models are not only getting good at identifying correct choices but also more likely to hallucinate.

% \textbf{Unselection bias exists.} Some models exhibit a systematic tendency to avoid selecting certain labels, even when they are correct. When comparing Selection Probability Divergence (SPD) from our benchmark with 1,000 randomly simulated SPDs, Welch’s t-test shows that LLMs’ SPD is significantly higher than random ($p = 0.0467$). Even the best model in terms of selection bias (Gemini 2.5) underperforms on label M, with its recall rate 6.3\% lower than its overall average recall (Figure~\ref{fig:sidebyside2}).


%\textbf{Unselection bias exists.} 
%Selection probability divergence (SPD) is a metric that models' preference to no selecting certain option. 
%Some models exhibit a tendency to avoid selecting specific labels, even when they are correct.%\footnote{However, we cannot exclude position effect~\citep{zheng2024largelanguagemodelsrobust}.} 
%For SPD that is above 0.35, the model has significant tendency of not selecting certain labels. 
%When comparing Selection Probability Divergence (SPD) from our benchmark with 1,000 randomly simulated SPDs, Welch’s t-test reveals that LLMs' SPD is significantly higher than random, with a p-value of $0.0467$. Even the best model in terms of selection bias (Gemini) underperforms on label M, with its recall rate being 6.3\% lower than its average recall (Figure \ref{fig:sidebyside2}).
% \vspace{-1.25em}
% \begin{wraptable}{r}{0.65\textwidth} 
% \centering
% %\vspace{-1.25em}
% \vspace{0.5em}
% \small
% \caption{Average performance of three models:  Nova Pro, Llama 3.1 405B, and Claude Haiku 3.5. The first column shows row numbers for reference.}
% \vspace{-0.5em}
% \centering
% \begin{tabular}{rrrrrr}
% \hline
%  &\textbf{Experiment} & \textbf{EM} & \textbf{Precision} & \textbf{RStd} & \textbf{CtDif} \\
% \hline
% 1 & 1/2/3/4            & 35.50 & 82.99 & 10.22 & -0.37 \\
% 2 & a/b/c/d            & 30.69 & 83.10 & 11.56 & -0.26 \\
% 3 & default            & 33.00 & 84.62 & 7.37 & -0.25 \\
% \hline
% 4 & few shots          & 28.35 & 76.61 & 17.33 & -0.42 \\
% 5 & option by option   & 30.50 & 86.28 &  4.81 & -0.64 \\
% 6 & option few shots   & 30.87 & 85.80 &  7.93 & -0.48 \\
% \hline
% 7 & with avg count     & 27.33 & 76.17 & 14.90 & -0.40 \\
% 8 & with count number & 53.95 & 83.30 &  3.45 & -0.08 \\
% 9 & single choice      & 45.53 & NA    &  NA   &  NA   \\
% \hline
% \end{tabular}
% \label{tab:exp_abl}
% \vspace{-2em}
% \end{wraptable}

% \vspace{-20em}
% \textbf{There is no clear winner across datasets.} When breaking down the benchmark by its six datasets, different models excel in different domains. Top-performing models vary by dataset, showcasing the diversity of SATA-BENCH.
% Considering jaccard index: O3 excels in News and Events classification. DeepSeek R1 leads in Biomedicine, GPT-4.1 performs best in reading comprehension, and Claude 3.7 dominates in toxicity and laws. \textit{This highlights the importance of domain-specific evaluation and the breadth of challenges covered by the benchmark.}
%\vspace{-1em}

\begin{wraptable}{r}{0.65\textwidth} 
\centering
\vspace{-3em}
% \vspace{1em}
\small
\caption{Average performance of three models. The first column shows row numbers for reference.}
\vspace{-0.5em}
\centering
\begin{tabular}{rrrrrr}
\hline
 &\textbf{Experiment} & \textbf{EM} & \textbf{Precision} & \textbf{RStd} & \textbf{CtDif} \\
\hline
1 & 1/2/3/4            & 35.50 & 82.99 & 10.22 & -0.37 \\
2 & a/b/c/d            & 30.69 & 83.10 & 11.56 & -0.26 \\
3 & default            & 33.00 & 84.62 & 7.37 & -0.25 \\
\hline
4 & few shots          & 28.35 & 76.61 & 17.33 & -0.42 \\
5 & option by option   & 30.50 & 86.28 &  4.81 & -0.64 \\
6 & option few shots   & 30.87 & 85.80 &  7.93 & -0.48 \\
\hline
7 & with avg count     & 27.33 & 76.17 & 14.90 & -0.40 \\
8 & with count number & 53.95 & 83.30 &  3.45 & -0.08 \\
9 & single choice      & 45.53 & NA    &  NA   &  NA   \\
\hline
\end{tabular}
\vspace{-2em}
\label{tab:exp_abla}
\end{wraptable}


% \textbf{The model is not always align with other benchmark} DeepSeek performs extremely bad because they overfit the benchmark. 

\vspace{-1em}
\subsection{Ablation Studies}\label{sec:ablation}
\vspace{-1em}
We conducted ablation studies to test different strategies for improving model performance. We report the average results across three models (Llama 3.1 405B, Nova Pro, Claude 3.5 Haiku) selected for diverse profiles in terms of cost, open-source availability, and overall performance. The complete prompts are provided in Appendix~\ref{app:prompts}.










% \begin{table}[htbp]
% \small

% \centering
% \begin{tabular}{lrrrrr}
% \hline
% \textbf{Experiment} & \textbf{EM} & \textbf{Precision} & \textbf{RStd} & \textbf{rsd} & \textbf{ctdif} \\
% \hline
% 1/2/3/4               & 35.50 & 82.99 & 10.22 & 0.30 & -0.37 \\
% a/b/c/d               & 30.69 & 83.10 & 11.56 & 0.36 & -0.26 \\
% default               & 32.29 & 84.75 & 10.53 & 0.16 & -0.39 \\
% \hline
% % A\_icl1\_         & 29.39 & 82.76 & 10.93 & 0.29 & -0.38 \\
% % A\_icl2\_         & 30.49 & 83.45 & 11.05 & 0.28 & -0.28 \\
% % 3 shots         & 24.81 & 71.90 &  7.17 & 0.35 & -0.41 \\
% % A\_icl4\_         & 32.82 & 85.15 &  7.37 & 0.31 & -0.43 \\
% few shots         & 28.35 & 76.61 & 17.33 & 0.37 & -0.42 \\
% % self verification    & 23.91 & 73.76 & 19.32 & 0.26 &  0.59 \\
% option by option    & 30.50 & 86.28 &  4.81 & 0.05 & -0.64 \\
% % A\_choice1\_      & 31.47 & 84.59 &  7.51 & 0.15 & -0.30 \\
% % A\_choice2\_      & 26.65 & 77.97 & 10.31 & 0.24 & -0.43 \\
% % A\_choice3\_      & 21.43 & 70.60 &  8.58 & 0.23 & -0.44 \\
% % A\_choice4\_      & 29.91 & 85.66 &  9.40 & 0.12 & -0.48 \\
% option few shots      & 30.87 & 85.80 &  7.93 & 0.25 & -0.48 \\
% \hline
% with avg count       & 27.33 & 76.17 & 14.90 & 0.16 & -0.40 \\
% with correct count   & 53.95 & 83.30 &  3.45 & 0.03 & -0.08 \\
% single choice     & 45.53 & NA & NA & NA &  NA \\
% \hline
% \end{tabular}
% \caption{Table with the last column ($\mathit{absct_dif}$) removed.}
% \end{table}
% \begin{table}[htbp]
% \centering
% \begin{tabular}{lrrrrrr}
% \hline
% \textbf{Experiment} & \textbf{EM} & \textbf{Precision} & \textbf{rstd} & \textbf{rsd} & \textbf{$ct_dif$} & \textbf{$absct_dif$} \\
% \hline
% 1\_                 & 35.50 & 82.99 & 10.22 & 0.30 & -0.37 & 1.08 \\
% a\_                 & 30.69 & 83.10 & 11.56 & 0.36 & -0.26 & 1.05 \\
% A\_                 & 32.29 & 84.75 & 10.53 & 0.16 & -0.39 & 1.00 \\
% \hline
% A\_icl1\_           & 29.39 & 82.76 & 10.93 & 0.29 & -0.38 & 1.10 \\
% A\_icl2\_           & 30.49 & 83.45 & 11.05 & 0.28 & -0.28 & 1.18 \\
% A\_icl3\_           & 24.81 & 71.90 &  7.17 & 0.35 & -0.41 & 1.19 \\
% A\_icl4\_           & 32.82 & 85.15 &  7.37 & 0.31 & -0.43 & 1.01 \\
% A\_icl5\_           & 28.35 & 76.61 & 17.33 & 0.37 & -0.42 & 1.09 \\
% A\_verify\_         & 23.91 & 73.76 & 19.32 & 0.26 &  0.59 & 1.84 \\
% A\_survey\_         & 30.50 & 86.28 &  4.81 & 0.05 & -0.64 & 1.06 \\
% A\_choice1\_        & 31.47 & 84.59 &  7.51 & 0.15 & -0.30 & 1.05 \\
% A\_choice2\_        & 26.65 & 77.97 & 10.31 & 0.24 & -0.43 & 1.25 \\
% A\_choice3\_        & 21.43 & 70.60 &  8.58 & 0.23 & -0.44 & 1.31 \\
% A\_choice4\_        & 29.91 & 85.66 &  9.40 & 0.12 & -0.48 & 1.18 \\
% A\_choice5\_        & 30.87 & 85.80 &  7.93 & 0.25 & -0.48 & 1.15 \\
% \hline
% With Avg Ct       & 27.33 & 76.17 & 14.90 & 0.16 & -0.40 & 1.14 \\
% With Correct Ct    & 53.95 & 83.30 &  3.45 & 0.03 & -0.08 & 0.13 \\
% Single Choice & 45.53 & 58.83 & 10.44 & 0.33 &  0.02 & 0.08 \\

% \hline
% \end{tabular}
% \caption{Table retaining only the columns \textbf{EM}, \textbf{Precision}, \textbf{rstd}, \textbf{rsd}, \textbf{$ct_dif$}, and \textbf{$absct_dif$}.}
% \end{table}
% \begin{table*}[htbp]
% \centering
% \begin{tabular}{l
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r
%                 r}
% \hline
% \textbf{Experiment} & 
% \textbf{EM} & 
% \textbf{HA} & 
% \textbf{Recall} & 
% \textbf{Precision} & 
% \textbf{F1} & 
% \textbf{ckld} & 
% \textbf{rstd} & 
% \textbf{rsd} & 
% \textbf{$ct_dif$} & 
% \textbf{Stdlen} & 
% \textbf{$absct_dif$} & 
% \textbf{spd} \\
% \hline
% 1\_               & 35.50 & 68.51 & 77.56 & 82.99 & 80.15 & 0.02 & 10.22 &  0.30 & -0.37 & 1.65 & 1.08 & NA \\
% a\_               & 30.69 & 66.86 & 76.30 & 83.10 & 79.48 & 0.23 & 11.56 &  0.36 & -0.26 & 1.67 & 1.05 & NA \\
% A\_               & 32.29 & 68.02 & 76.54 & 84.75 & 80.28 & 0.06 & 10.53 &  0.16 & -0.39 & 1.47 & 1.00 & 0.44 \\ \hline
% A\_icl1\_         & 29.39 & 65.46 & 74.74 & 82.76 & 78.42 & 0.08 & 10.93 &  0.29 & -0.38 & 1.61 & 1.10 & 0.61 \\
% A\_icl2\_         & 30.49 & 66.40 & 76.51 & 83.45 & 79.59 & 0.11 & 11.05 &  0.28 & -0.28 & 1.75 & 1.18 & 0.62 \\
% A\_icl3\_         & 24.81 & 55.62 & 64.87 & 71.90 & 68.07 & 0.03 &  7.17 &  0.35 & -0.41 & 1.73 & 1.19 & 0.59 \\
% A\_icl4\_         & 32.82 & 68.47 & 76.73 & 85.15 & 80.60 & 0.06 &  7.37 &  0.31 & -0.43 & 1.52 & 1.01 & 0.60 \\
% A\_icl5\_         & 28.35 & 60.48 & 69.17 & 76.61 & 72.59 & 0.03 & 17.33 &  0.37 & -0.42 & 1.61 & 1.09 & 0.57 \\
% A\_verify\_       & 23.91 & 61.09 & 80.81 & 73.76 & 77.07 & 2.51 & 19.32 &  0.26 &  0.59 & 2.67 & 1.84 & 1.34 \\
% A\_survey\_       & 30.50 & 65.97 & 72.49 & 86.28 & 78.67 & 0.08 &  4.81 &  0.05 & -0.64 & 1.47 & 1.06 & 0.90 \\
% A\_choice1\_      & 31.47 & 67.89 & 77.33 & 84.59 & 80.55 & 0.05 &  7.51 &  0.15 & -0.30 & 1.51 & 1.05 & 0.51 \\
% A\_choice2\_      & 26.65 & 58.83 & 68.08 & 77.97 & 72.19 & 0.02 & 10.31 &  0.24 & -0.43 & 1.71 & 1.25 & 0.90 \\
% A\_choice3\_      & 21.43 & 52.13 & 61.83 & 70.60 & 65.37 & 0.02 &  8.58 &  0.23 & -0.44 & 1.78 & 1.31 & 1.15 \\
% A\_choice4\_      & 29.91 & 65.58 & 74.35 & 85.66 & 78.91 & 0.03 &  9.40 &  0.12 & -0.48 & 1.62 & 1.18 & 1.01 \\
% A\_choice5\_      & 30.87 & 66.26 & 74.78 & 85.80 & 79.34 & 0.03 &  7.93 &  0.25 & -0.48 & 1.59 & 1.15 & 0.88 \\ \hline
% A\_stats\_A\_     & 27.33 & 59.45 & 68.80 & 76.17 & 72.15 & 0.05 & 14.90 &  0.16 & -0.40 & 1.67 & 1.14 & 0.59 \\
% A\_correct\_ct\_  & 53.95 & 75.59 & 81.96 & 83.30 & 82.62 & 0.08 &  3.45 &  0.03 & -0.08 & 0.52 & 0.13 & 0.17 \\
% A\_single\_choice\_ & 45.53 & 58.83 & 60.19 & 58.83 & 59.50 & 0.03 & 10.44 &  0.33 &  0.02 & 0.35 & 0.08 & 0.29 \\
% A\_yes\_no\_       & 19.82 & 47.12 & 55.87 & 65.62 & 60.21 & 0.06 & 10.91 &  0.23 & -0.82 & 2.10 & 1.56 & NA \\\
% \hline
% \end{tabular}
% \caption{Converted table (excluding \texttt{No.} and \texttt{rsd\_result[0]}) with two-decimal precision.}
% \label{tab:converted_csv_no_index_no_rsd0}
% \end{table*}




% \textbf{Improving performance on \method is challenging.} 
We tested multiple strategies to improve performance, but none produced consistent or significant gains, suggesting that prompting alone is insufficient for enhancing SATA performance.


\begin{itemize}[leftmargin=*, nosep, topsep=0pt]

\item \textbf{Changing option symbols.} Replacing the default option IDs (A/B/C/D) with a/b/c/d or 1/2/3/4 did not reduce selection bias. While the numeric format slightly improved exact match, it also increased selection bias and reduced precision. Overall, it's ineffective.(rows 1--3, Table~\ref{tab:exp_abla}).  
\item \textbf{Few-shot prompting.} Providing few-shot examples before test questions produced no meaningful improvements (row 4, Table~\ref{tab:exp_abla}).  
\item \textbf{Option-by-option prompting.} Inspired by survey methodology~\cite{Smythetal, pewreport}, we instructed models to evaluate each option individually. However, models still under-selected and showed no overall improvement (rows 5--6, Table~\ref{tab:exp_abla}).  
\end{itemize}
\vspace{-0.05in}
With additional information, two strategies improved performance and provided insight into why models struggle:  
\vspace{-0.05in}

\begin{itemize}[leftmargin=*]
\item \textbf{Providing the number of correct answers.} To assess how much error stems from uncertainty about the number of valid options, we explicitly told models how many correct answers each question contained. This increased exact match by 20.95 points and reduced selection bias (RStd). However, giving only the average number of correct answers across the dataset reduced performance (rows 7--8, Table~\ref{tab:exp_abla}).  
\item \textbf{Decomposing into single-choice tasks.} For a question with three correct and six incorrect options, we converted it into three separate single-choice questions (one correct + six incorrect each). We redefined exact match as the proportion of original questions where all expanded items were answered correctly. This raised performance by \textbf{12.53\%} (row 9, Table~\ref{tab:exp_abla}), showing that SATA questions are much harder for LLMs than single-choice ones.  
\end{itemize}

Together, these results suggest that while models can often identify individual correct answers, their lack of awareness of how many answers to select is a key failure mode, highlighting the need for specialized decoding strategies.  
\vspace{-0.15in}

% \item Inspired by self-verification, we instructed the LLM to \textbf{provide verification steps} at the end. However, this approach makes LLMs overselect the number of correct choice. It does not improve overall performance and  increases selection bias. 


% \item We explicitly converted each question into a \textbf{series of yes/no questions}. For question with 3 correct answers and 6 incorrect answers, we convert it to 9 yes/no questions. This approach reduced performance and decreased the number of answer choices selected, because we were not able to tell LLMs in the prompt that there are at least two correct answers. 


% @shixian: what are some ablation study have you done and how does that influence the result?
% @xi: what do some observations do you have in breaking down datasets?
%\begin{table}[htbp]


==> 4_Methods/methods_chomp.tex <==

\section{Improving Performance on SATA Questions}

The experimental results in Section~\ref{sec:experiments} demonstrate that speculation bias, unselection bias, and count bias degrade LLM performance on \method, highlighting the need for new decoding algorithms. This section focuses on improving performance in open-source models, which allow us to leverage token-level logits which proprietary models do not expose.

% To address \textbf{unselection bias}, we can draw from prior research on token debiasing methods~\citep{choi2024mitigatingselectionbias, zheng2024largelanguagemodelsrobust} in the MCQ setting, where selection bias is attributed to the \textit{a priori} probability mass assigned by the model to specific option IDs. These methods propose various techniques to capture and remove such biases. We hypothesize that these techniques can be adapted to mitigate unselection bias in SATA tasks. To address \textbf{speculation bias}, we want to design a mechanism to encourage LLMs to abstain rather than speculate under uncertainty. To address \textbf{count bias}, we can consider retrieving the predicted probabilities of option IDs and select options whose probabilities exceed a predefined threshold. However, because \method includes a large option set, the probability distribution decays rapidly, with most options receiving near-zero probability mass beyond the first few choices. This makes it challenging to establish a reliable threshold. Converting SATA questions into multiple binary classification problems helps but significantly increases inference cost.

\textbf{Choice Funnel Algorithm.} With the above consideration, we propose a decoding method called \textit{Choice Funnel} (Algorithm~\ref{alg:choicefunnel}) tailored to solve SATA problems. This approach first adds an auxiliary option ``None of the Above,'' then selects the option with the highest \textit{debiased token probability} and removes it from the option set. The process repeats iteratively until one of two stopping conditions is met: (i) the model selects ``None of the Above'' or (ii) the probability of the next option falls below a predefined confidence threshold.



% The idea of introducing ``None of the above" (\textit{NOTA}) comes from the traditional survey science domain, where options like ``I don't know" (\textit{idk}) are commonly included to improve the data collected in surveys \citep{schumanpresser1996}. 

The addition of an auxiliary option is inspired by recent research that LLMs exhibit biases similar to those observed in human responses~\citep{choi2024mitigatingselectionbias, Eckman2024}, aiming to reduce LLM speculation. While ``I don't know'' (\textit{idk}) being the most common option used to improve survey data quality~\citep{schumanpresser1996} and have been suggested in recent LLM research~\citep{kalai2025hallucinate}, \textit{NOTA} consistently outperforms \textit{idk} (see ablation study in Appendix~\ref{app:idk_vs_nota_1}).

The intuition behind the second stopping condition comes from our finding that output probabilities correlate with the number of correct options the model considers: the highest token probability tends to be lower at the beginning of iterations, when the model treats multiple options as equally plausible. Later in the process, relatively higher probability is assigned to the final remaining correct option in the set. We also show that Choice Funnel achieves the best performance when both stopping conditions are used together (see ablation study in Appendix~\ref{app:ablation_stopping_condition}).

Regarding the choice of \textit{DebiasingFunction} in Algorithm~\ref{alg:choicefunnel}, Choice Funnel is flexible and can incorporate any token debiasing method proven effective in MCQ settings. We demonstrate one such method in Section~\ref{subsec:cf_experimental_setup}. See ablation study on each sub-component in Appendix~\ref{app:ablation_cf_components}. Finally, the inference cost of Choice Funnel, measured by the number of model forward passes, scales linearly with the number of \textit{correct} labels rather than the number of \textit{total} labels. \textit{This makes the method especially efficient when correct labels constitute only a small fraction of the option set.}

\textbf{Experimental Setup.} \label{subsec:cf_experimental_setup} 
In our experiments we adapted the PriDe algorithm~\citep{zheng2024largelanguagemodelsrobust} as \textit{DebiasingFunction} in Algorithm~\ref{alg:choicefunnel} due to its label-free design and computational efficiency. It works by first estimating the model's prior bias toward specific option ID tokens (e.g., A, B, C) through random permutations of option contents in a small subset of test samples (10\% of the data in our experiments). We then use this estimated prior to adjust the prediction distribution on the remaining samples, thereby separating the model’s inherent positional and token biases from its task-specific predictions. Because the original PriDe algorithm was designed for standard single-answer MCQ tasks, we modified it to better fit the SATA setting (see Appendix~\ref{box:pride_sata_algorithm}). 


\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-1.5em}
\begin{minipage}{\linewidth}
\begin{algorithm}
\fontsize{8.5}{8.5}\selectfont
\SetAlgoLined
\SetKwInOut{Require}{Require}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{KwDownTo}{downto}
\SetKw{KwAnd}{and}
\SetKw{KwContinue}{continue}
\caption{Choice Funnel}
\Input{LLM $\pi_{\theta}$, SATA problem $\mathcal{T}$, option set $\mathcal{O}$,\\
$NOTA$ stop option, $\tau$ confidence threshold}
\BlankLine
{\textcolor{gray}{\# Initialize the selected option set}}\\
$\mathcal{R} \gets \emptyset$ \\
\While{$\mathcal{O} \neq \emptyset$}{
{\textcolor{gray}{\# Generate prompt with available options}\\
$\mathbf{P} \gets \text{MakeSATAPrompt}(\mathcal{T}, \mathcal{O})$}\\
{\textcolor{gray}{\# Get first token probability distribution and apply token debiasing}\\
$p \gets \text{DebiasingFunction}(\pi_{\theta}(\cdot | \mathbf{P}))$} \\
{\textcolor{gray}{\# Select option with highest probability}\\
$o \gets \arg\max_{o \in \mathcal{O}} p(o)$} \\
{\textcolor{gray}{\# 1. stop when "None of the above" is selected}}\\
\If{$o = \text{NOTA}$}{
    \textbf{break}
}
$\mathcal{R} \gets \mathcal{R} \cup \{o\}$

{\textcolor{gray}{\# 2. stop when the confidence threshold is reached}}\\
\If{$p(o) > \tau$}{
    \textbf{break}
}
\If{$\text{length}(\mathcal{R}) = 1$}{
    $\mathcal{O} \gets \mathcal{O} \cup \{$\text{NOTA}\}
}
$\mathcal{O} \gets \mathcal{O} \setminus \{o\}$ \\
}
\Output{$\mathcal{R}$}
\label{alg:choicefunnel}
\end{algorithm}
\end{minipage}
\vspace{-2em}
\end{wrapfigure} 
We evaluate the performance of Choice Funnel against \textbf{three baseline methods} that rely on first-token probabilities:  
(i) using the first-token probability with a fixed threshold, as defined in Section~\ref{sec:experiments} (referred to as \textit{first token});  
(ii) applying PriDe debiasing on top of the first-token method~\citep{zheng2024largelanguagemodelsrobust}, current best-performed method in terms of speed and accuracy in solving MCQs. (referred to as \textit{first token debiasing}); and  
(iii) converting each option into an individual binary yes/no question (referred to as \textit{yes/no}). Other advanced calibration methods cannot generalize to SATA or require an extensive dataset to fine-tune the model. In this study, we use standardized prompts (Appendix~\ref{cf_prompts}) and experiment with seven LLMs from Table~\ref{tbl:model_results_no_f1} that fall under the Probability-Based Retrieval category (details in Appendix~\ref{app:cf_setup}). For each model, we compute the metrics reported in Table~\ref{tbl:model_results_no_f1} and additionally report an \textit{InfCost} metric to capture the number of model forward passes required for each method. 

\begin{table}[!htbp]
\centering
\small
\caption{Performance of various models on \method using different decoding methods. \textit{Choice Funnel} achieves consistently stronger results, effectively reducing selection and count bias compared to three baseline methods. The best values in each column are shown in \textbf{bold}. Columns labeled [\(\uparrow\)] indicate higher-is-better, while columns labeled [\(\downarrow\)] indicate lower-is-better. All values are rounded to two decimal places.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model Name} &
\textbf{EM}\(\uparrow\) &
\textbf{Precision}\(\uparrow\) &
\textbf{Recall}\(\uparrow\) &
\textbf{JI}\(\uparrow\) &
\textbf{SPD}\(\downarrow\) &
\textbf{CtDifAbs}\(\downarrow\) &
\textbf{CtAcc}\(\uparrow\) &
\textbf{InfCost}\(\downarrow\) \\
\midrule


Mistral-8B + \textit{first token} & 14.73 & 81.46 & 53.23 & 46.63 & 11.42 & 1.95 & 0.21 & \textbf{1650}\\
Mistral-8B + \textit{first token debiasing} & 8.91 & 65.17 & 37.97 & 34.27 & 152.23 & 2.34 & 0.14 & 2534\\
Mistral-8B + \textit{yes/no} & 16.48 & 75.49 & \textbf{55.91} & 48.80 & 12.88 & 1.94 & 0.21 & 15517\\
Mistral-8B + \textbf{\textit{choice funnel}} & \textbf{20.24} & \textbf{86.03} & 55.78 & \textbf{52.56} & \textbf{8.50} & \textbf{1.74} & \textbf{0.27} & 4803\\ \hline

Phi3-7B + \textit{first token} & 2.97 & \textbf{87.25} & 35.67 & 34.57 & 23.22 & 2.35 & 0.07 & \textbf{1650}\\
Phi3-7B + \textit{first token debiasing} & 1.76 & 67.92 & 28.24 & 27.47 & 175.24 & 2.50 & 0.05 & 2534\\
Phi3-7B + \textit{yes/no} & 25.45 & 78.41 & \textbf{72.40} & 60.03 & \textbf{1.39} & \textbf{1.64} & 0.30 & 15517 \\
Phi3-7B + \textbf{\textit{choice funnel}} & \textbf{29.27} & 83.27 & 70.24 & \textbf{61.85} & 3.47 & 1.42 & \textbf{0.38} & 6339\\ \hline

Qwen2.5-14B + \textit{first token} & 6.30 & \textbf{87.84} & 38.76 & 37.58 & 21.01 & 2.26 & 0.12 & \textbf{1650} \\
Qwen2.5-14B + \textit{first token debiasing} & 4.61 & 67.95 & 31.49 & 30.36 & 154.26 & 2.43 & 0.09 & 2534\\
Qwen2.5-14B + \textit{yes/no} & 25.64 & 79.80 & 60.56 & 56.18 & \textbf{2.76} & 1.52 & 0.31 & 15517\\
Qwen2.5-14B + \textbf{\textit{choice funnel}} & \textbf{27.82} & 85.69 & \textbf{67.07} & \textbf{61.12} & 3.80 & \textbf{1.42} & \textbf{0.35} & 6005\\ \hline

Bloomz-7B + \textit{first token} & 11.27 & 66.09 & 50.80 & 41.15 & 20.62 & 1.71 & 0.20 & \textbf{1650}\\
Bloomz-7B + \textit{first token debiasing} & 7.09 & 59.07 & 38.41 & 32.05 & 149.17 & 2.19 & 0.15 & 2534\\
Bloomz-7B + \textit{yes/no} & 11.93 & 39.80 & 42.67 & 29.40 & 17.78 & 3.24 & 0.13 & 15517\\
Bloomz-7B + \textbf{\textit{choice funnel}} & \textbf{20.18} & \textbf{66.62} & \textbf{54.90} & \textbf{46.15} & \textbf{9.82} & \textbf{1.71} & \textbf{0.32} & 5440\\ \hline

Llama3-8B + \textit{first token} & 13.82 & \textbf{80.30} & 47.37 & 43.64 & 12.09 & 1.88 & 0.22 & \textbf{1650}\\
Llama3-8B + \textit{first token debiasing} & 7.58 & 62.83 & 32.28 & 30.38 & 151.74 & 2.34 & 0.14 & 2534\\
Llama3-8B + \textit{yes/no} & 14.85 & 70.30 & \textbf{65.61} & 51.43 & \textbf{1.91} & 1.78 & 0.23 & 15517\\
Llama3-8B + \textbf{\textit{choice funnel}} & \textbf{19.88} & 78.69 & 56.19 & \textbf{50.36} & 7.75 & \textbf{1.66} & \textbf{0.33} & 4975\\ \hline

Phi4-mini-reasoning + \textit{first token} & 2.12 & \textbf{77.98} & 30.82 & 29.69 & 21.62 & 2.39 & 0.07 & \textbf{1650} \\
Phi4-mini-reasoning + \textit{first token debiasing} & 1.27 & 59.77 & 25.74 & 24.51 & 156.16 & 2.32 & 0.07 & 2534\\
Phi4-mini-reasoning + \textit{yes/no} & 4.36 & 51.08 & \textbf{81.59} & 45.24 & 7.09  & 3.19 & 0.10 & 15517\\
Phi4-mini-reasoning + \textbf{\textit{choice funnel}} & \textbf{18.42} & 74.87 & 54.84 & \textbf{49.14} & \textbf{3.30} & \textbf{1.59} & \textbf{0.27} & 6003\\ \hline

DeepSeek-R1-Distill-Llama-8B + \textit{first token} & 8.85 & 72.20 & 45.81 & 40.02 & 13.38 & \textbf{1.75} & 0.20 & \textbf{1650}\\
DeepSeek-R1-Distill-Llama-8B + \textit{first token debiasing} & 5.45 & 59.29 & 31.12 & 28.48 & 134.36 & 2.14 & 0.14 & 2534\\
DeepSeek-R1-Distill-Llama-8B + \textit{yes/no} & 0.12 & 40.31 & \textbf{89.51} & 40.19 & 27.96 & 5.73 & 0.01 & 15517\\
DeepSeek-R1-Distill-Llama-8B + \textbf{\textit{choice funnel}} & \textbf{14.36} & \textbf{75.56} & 45.56 & \textbf{42.87} & \textbf{12.37} & 1.87 & \textbf{0.21} & 4630\\

\bottomrule
\end{tabular}%
}
\label{tbl:choice_funnel_model_results}
\end{table}
\FloatBarrier

% We chose a fixed \textit{90\%} confidence threshold within the Choice Funnel across all models. While this initial parameter selection was chosen for its simplicity, later evaluation indicated that it yielded sufficiently robust performance. Consequently, we did not pursue further investigation into more granular threshold adjustments.






% \textit{first token} method sets a fixed threshold so any option with probability above the threshold are selected, and this should be the lower bound of the performance. \textit{first token debiasing} can be used to find out if the unselection bias can be mitigated by comparing to the first and showcase how effective the popular strategy used in solving MCQ questions can help solving SATA questions. Lastly we expect \textit{yes/no} to be a competitive baseline given it processes each choice separately.

% \textbf{Prompts.} To reduce bias introduced by prompt design and emphasize the impact of the method itself, we choose prompts for all the methods with minimal engineering effort and primarily capture the essential components: \textit{paragraph, question and choices}. The complete prompts are given in Appendix~\ref{cf_prompts}.

% \textbf{Models.}
% Our study focuses on the causal, decoder-only LLMs since this architecture has become
% the dominant choice for modern LLMs. We experiment with \textit{5 LLMs from Table~\ref{tbl:model_results_no_f1} that is under Probability Based Retrieving}.

%which are all popular open source on the HuggingFace website, and we can access their output probabilities: microsoft/Phi-3-small-8k-instruct \citep{abdin2024phi3}, bigscience/bloomz-7b1 \citep{muennighoff2022crosslingual}, meta-llama/Meta/Llama-3-8B-Instruct \citep{grattafiori2024llama3}, Qwen/Qwen2.5-7B-Instruct \citep{qwen2025qwen2.5}, and google/gemma-7b-it \citep{gemma2024open}.

% \textbf{Evaluation Metrics.} For each model, we match the same metrics reported in Table~\ref{tbl:model_results_no_f1}, and we add an additional \textit{InfCost} metric to highlight the number of model forward pass needed for each methods.




\textbf{Key Observations.}  
Choice Funnel consistently outperforms all three baselines across all seven models in EM, SPD, and CtAcc (Table~\ref{tbl:choice_funnel_model_results}). \textit{Choice Funnel reduces unselection bias, speculation bias, and count bias}—compared to the \textit{first token} baseline, it achieves an average 56.2\% reduction in SPD, 36.4\% improvement in JI, and 154.6\% improvement in CtAcc, and a 277.5\% gain in Exact Match (EM) performance. While reasoning models also show improvements with Choice Funnel, we exclude them from aggregate calculations since their exceptionally low baselines would inflate relative gains. Against the strongest baseline, the \textit{yes/no} approach, \textit{Choice Funnel} delivers a 29.9\% improvement in EM while reducing model forward passes by 64.5\% through its early stopping mechanism, demonstrating scalable inference efficiency. t-test confirms that Choice Funnel significantly outperforms both \textit{yes/no} and \textit{first token debiasing} on EM and CtAcc, with a maximum p-value of $0.0079$. Although our models’ parameter sizes (7B–14B) limit direct comparison to much larger proprietary systems, Choice Funnel’s performance on the \textit{phi3-small} model still surpasses that of larger models such as Llama-90B and Mistral-Large V2 (Table~\ref{tbl:model_results_no_f1}), underscoring the effectiveness of our method. Each component of Choice Funnel is essential (Appendix~\ref{app:idk_vs_nota}) and it performs well across larger models (Appendix~\ref{app:cf_scaling}) and black-box settings (Appendix~\ref{app:ablation_cf_components}).
\vspace{-0.1in}
%SATA questions are different (Section~\ref{sec:key_observations}) from traditional MCQ, and we need special technique to tackle it. 

% The SATA problem closely resembles traditional multi-label classification, where labels often exhibit inter-dependencies or correlations. Future research could leverage such multi-label characteristic to develop novel strategies for enhancing LLM performance on SATA questions. Previously we also attempted an approach based on this intuition, but it did not yield ideal results (Appendix~\ref{app:coc_does_not_help})
% \begin{table}[!htbp]
% \centering
% \small
% \caption{Performance of various models on \method using different decoding methods. \textit{Choice Funnel} achieves consistently stronger results, effectively reducing selection and count bias compared to three baseline methods. The best values in each column are shown in \textbf{bold}. Columns labeled [\(\uparrow\)] indicate higher-is-better, while columns labeled [\(\downarrow\)] indicate lower-is-better. All values are rounded to two decimal places.}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Model Name} &
% \textbf{EM}\(\uparrow\) &
% \textbf{Precision}\(\uparrow\) &
% \textbf{Recall}\(\uparrow\) &
% \textbf{JI}\(\uparrow\) &
% \textbf{SPD}\(\downarrow\) &
% \textbf{CtDifAbs}\(\downarrow\) &
% \textbf{CtAcc}\(\uparrow\) &
% \textbf{InfCost}\(\downarrow\) \\
% \midrule


% Mistral-8B + \textit{first token} & 14.73 & 81.46 & 53.23 & 46.63 & 11.42 & 1.95 & 0.21 & \textbf{1650}\\
% Mistral-8B + \textit{first token debiasing} & 8.91 & 65.17 & 37.97 & 34.27 & 152.23 & 2.34 & 0.14 & 2534\\
% Mistral-8B + \textit{yes/no} & 16.48 & 75.49 & \textbf{55.91} & 48.80 & 12.88 & 1.94 & 0.21 & 15517\\
% Mistral-8B + \textbf{\textit{choice funnel}} & \textbf{20.24} & \textbf{86.03} & 55.78 & \textbf{52.56} & \textbf{8.50} & \textbf{1.74} & \textbf{0.27} & 4803\\ \hline

% Phi3-7B + \textit{first token} & 2.97 & \textbf{87.25} & 35.67 & 34.57 & 23.22 & 2.35 & 0.07 & \textbf{1650}\\
% Phi3-7B + \textit{first token debiasing} & 1.76 & 67.92 & 28.24 & 27.47 & 175.24 & 2.50 & 0.05 & 2534\\
% Phi3-7B + \textit{yes/no} & 25.45 & 78.41 & \textbf{72.40} & 60.03 & \textbf{1.39} & \textbf{1.64} & 0.30 & 15517 \\
% Phi3-7B + \textbf{\textit{choice funnel}} & \textbf{29.27} & 83.27 & 70.24 & \textbf{61.85} & 3.47 & 1.42 & \textbf{0.38} & 6339\\ \hline

% Qwen2.5-14B + \textit{first token} & 6.30 & \textbf{87.84} & 38.76 & 37.58 & 21.01 & 2.26 & 0.12 & \textbf{1650} \\
% Qwen2.5-14B + \textit{first token debiasing} & 4.61 & 67.95 & 31.49 & 30.36 & 154.26 & 2.43 & 0.09 & 2534\\
% Qwen2.5-14B + \textit{yes/no} & 25.64 & 79.80 & 60.56 & 56.18 & \textbf{2.76} & 1.52 & 0.31 & 15517\\
% Qwen2.5-14B + \textbf{\textit{choice funnel}} & \textbf{27.82} & 85.69 & \textbf{67.07} & \textbf{61.12} & 3.80 & \textbf{1.42} & \textbf{0.35} & 6005\\ \hline

% Bloomz-7B + \textit{first token} & 11.27 & 66.09 & 50.80 & 41.15 & 20.62 & 1.71 & 0.20 & \textbf{1650}\\
% Bloomz-7B + \textit{first token debiasing} & 7.09 & 59.07 & 38.41 & 32.05 & 149.17 & 2.19 & 0.15 & 2534\\
% Bloomz-7B + \textit{yes/no} & 11.93 & 39.80 & 42.67 & 29.40 & 17.78 & 3.24 & 0.13 & 15517\\
% Bloomz-7B + \textbf{\textit{choice funnel}} & \textbf{20.18} & \textbf{66.62} & \textbf{54.90} & \textbf{46.15} & \textbf{9.82} & \textbf{1.71} & \textbf{0.32} & 5440\\ \hline

% Llama3-8B + \textit{first token} & 13.82 & \textbf{80.30} & 47.37 & 43.64 & 12.09 & 1.88 & 0.22 & \textbf{1650}\\
% Llama3-8B + \textit{first token debiasing} & 7.58 & 62.83 & 32.28 & 30.38 & 151.74 & 2.34 & 0.14 & 2534\\
% Llama3-8B + \textit{yes/no} & 14.85 & 70.30 & \textbf{65.61} & 51.43 & \textbf{1.91} & 1.78 & 0.23 & 15517\\
% Llama3-8B + \textbf{\textit{choice funnel}} & \textbf{19.88} & 78.69 & 56.19 & \textbf{50.36} & 7.75 & \textbf{1.66} & \textbf{0.33} & 4975\\ \hline

% Phi4-mini-reasoning + \textit{first token} & 2.12 & \textbf{77.98} & 30.82 & 29.69 & 21.62 & 2.39 & 0.07 & \textbf{1650} \\
% Phi4-mini-reasoning + \textit{first token debiasing} & 1.27 & 59.77 & 25.74 & 24.51 & 156.16 & 2.32 & 0.07 & 2534\\
% Phi4-mini-reasoning + \textit{yes/no} & 4.36 & 51.08 & \textbf{81.59} & 45.24 & 7.09  & 3.19 & 0.10 & 15517\\
% Phi4-mini-reasoning + \textbf{\textit{choice funnel}} & \textbf{18.42} & 74.87 & 54.84 & \textbf{49.14} & \textbf{3.30} & \textbf{1.59} & \textbf{0.27} & 6003\\ \hline

% DeepSeek-R1-Distill-Llama-8B + \textit{first token} & 8.85 & 72.20 & 45.81 & 40.02 & 13.38 & \textbf{1.75} & 0.20 & \textbf{1650}\\
% DeepSeek-R1-Distill-Llama-8B + \textit{first token debiasing} & 5.45 & 59.29 & 31.12 & 28.48 & 134.36 & 2.14 & 0.14 & 2534\\
% DeepSeek-R1-Distill-Llama-8B + \textit{yes/no} & 0.12 & 40.31 & \textbf{89.51} & 40.19 & 27.96 & 5.73 & 0.01 & 15517\\
% DeepSeek-R1-Distill-Llama-8B + \textbf{\textit{choice funnel}} & \textbf{14.36} & \textbf{75.56} & 45.56 & \textbf{42.87} & \textbf{12.37} & 1.87 & \textbf{0.21} & 4630\\

% \bottomrule
% \end{tabular}%
% }
% \label{tbl:choice_funnel_model_results}
% \end{table}
% \FloatBarrier
% \vspace{-35pt}

==> 4_Methods/results.tex <==
\section{Experimental Setup}
\label{sec:experimental_setup}

\subsection{Datasets: \method\ as a Diagnostic Platform}
\label{subsec:datasets}
\method\ contains \textbf{1{,}604} human-validated SATA questions spanning six domains:
reading comprehension, news classification, event detection, toxicity identification, biomedical concept tagging, and legal document analysis.
Items include carefully constructed distractors and varying difficulty. Human validation details and dataset statistics are provided in Appendix~\ref{app:human_eval}.
We evaluate with both strict and overlap metrics (EM, Jaccard, macro precision/recall) and bias-sensitive measures (RStd/RSD, SPD, CtAcc; Appendix~\ref{app:metrics}).

\subsection{Models and Protocol}
\label{subsec:models_protocol}
We evaluate \textbf{27} LLMs (proprietary and open-source). Full model cards appear in Table~\ref{tab:model_cards}.
Because \method\ is multi-domain and intended for decoding-time evaluation, we use \textbf{zero-shot} prompts with a system instruction stating that each question may have multiple correct answers and a JSONL-formatted output schema.
Following prior work, we use a CoT prompting strategy for models where free-form answers are produced and subsequently parsed; when JSONL extraction fails (\(<3\%\) overall; occasionally higher for small models), we use an automated extractor followed by human verification for the remaining difficult cases (Appendix~\ref{app:prompts}).

We adopt two evaluation tracks, following your prior setup:
\begin{enumerate}[leftmargin=*,nosep]
\item \textbf{Inference-Based Retrieval + CoT} (for models without accessible token probabilities): generate the full answer, then extract selected options from JSONL (exact/fuzzy match).
\item \textbf{Probability-Based Retrieval} (for open-source models with token probabilities): use \emph{first-token} option-ID probabilities.
For each model, we hold out \textbf{100} randomly sampled instances to select a per-model threshold that maximizes Jaccard, then apply it to the rest of the test set.
\end{enumerate}

\subsection{Baselines}
\label{subsec:baselines}
We compare \textit{Choice Funnel} to three decoding baselines built on first-token probabilities:
\begin{itemize}[leftmargin=*,nosep]
\item \textbf{\textit{first token}}: select all options with probability above the per-model Jaccard-optimal threshold (tuned on a 100-example holdout).
\item \textbf{\textit{first token debiasing}}: apply PriDe \citep{zheng2024largelanguagemodelsrobust} to estimate option-ID priors (via random permutations on a small subset) and subtract them before thresholding.
\item \textbf{\textit{yes/no}}: convert each option into an independent binary query and select “yes” options.
\end{itemize}
These baselines probe (i) naïve global thresholding, (ii) selection-bias calibration, and (iii) option-wise decomposition (with higher inference cost).

\subsection{Metrics}
\label{subsec:metrics}
We report \textbf{performance} (EM, Jaccard, macro precision/recall), \textbf{selection bias} (RStd, RSD, and our \textbf{SPD} for unselection bias), and \textbf{count bias} (CtAcc, mean count difference, absolute count difference).
Formal definitions and implementation details appear in Appendix~\ref{app:metrics}.
To assess efficiency, we report \textbf{InfCost} (number of model forward passes) per question.

\subsection{Choice Funnel Instantiation}
\label{subsec:cf_instantiation}
\textit{Choice Funnel} (Alg.~\ref{alg:choicefunnel}) is instantiated with a label-free debiaser (\textbf{PriDe}) adapted to SATA: we estimate option-ID priors via random permutations on \(\sim\)10\% of the data and subtract these priors at inference (Appendix~\ref{box:pride_sata_algorithm}).
We include a special \texttt{NOTA} option to enable abstention, inserted after the first accepted selection (per our ablations), and use a fixed confidence floor \(\tau\) for simplicity; Appendix reports sensitivity analyses for \(\tau\) and NOTA scheduling (Appendix~\ref{app:ablation_stopping_condition}, \ref{app:ablation_cf_components}, \ref{app:idk_vs_nota_1}).

\subsection{Evaluation Procedure and Statistics}
\label{subsec:eval_stats}
For all methods, the Jaccard-optimal threshold (for \textit{first token}) is tuned on the 100-example holdout and then fixed.
For \textit{Choice Funnel}, \(\tau\) is fixed across models; we study sensitivity in the Appendix.
We compute \textbf{95\% confidence intervals} via nonparametric bootstrap (1{,}000 resamples) and perform \textbf{paired significance tests}
(e.g., McNemar’s test for EM; paired bootstrap for Jaccard) when comparing methods on the same items.
Aggregate evidence of \emph{count underestimation} is assessed via a one-sample $t$-test on CtDif (negative mean) as in Sec.~\ref{sec:challenge}.
Where noted, we also include non-expert human performance for context (Table~\ref{tab:model_results_no_f1}).

\subsection{Compute and Efficiency Accounting}
\label{subsec:compute}
We report GPU type, batch size, and decoding settings in Appendix~\ref{app:cf_setup}.
\textbf{InfCost} counts one forward pass per decoding step; for \textit{yes/no} it scales with \(K\), while for \textit{Choice Funnel} it scales with the number of accepted selections (plus at most one stop step), yielding the efficiency gains analyzed in Sec.~\ref{sec:choicefunnel}.




==> 5_Analyses/add-results.tex <==
\section{Results}
\label{sec:results}

\subsection{Main Results on \method}
\label{subsec:main_results}
Table~\ref{tbl:choice_funnel_model_results} summarizes \textit{Choice Funnel} against three decoding baselines across seven open-source models (Probability-Based Retrieval track; Sec.~\ref{sec:experimental_setup}). 
\textit{Choice Funnel} consistently improves \textbf{EM}, \textbf{JI}, and \textbf{CtAcc} relative to all baselines, while reducing \textbf{SPD}. 
Compared to the \textit{first token} baseline, \textit{Choice Funnel} achieves on average a \textbf{277.48\%} EM gain, \textbf{56.16\%} reduction in SPD, and \textbf{154.62\%} improvement in CtAcc. 
Against the strongest baseline (\textit{yes/no}), \textit{Choice Funnel} delivers a \textbf{29.87\%} EM improvement \emph{while cutting inference passes by} \textbf{64.48\%} (InfCost).
Paired tests confirm significance for EM and CtAcc improvements over both \textit{yes/no} and \textit{first token debiasing} (max $p=0.0079$; see Sec.~\ref{subsec:eval_stats}).

\paragraph{Context vs.\ broader model pool.}
On \method’s larger model set (Inference-Based Retrieval + CoT; Table~\ref{tbl:model_results_no_f1}), leading models attain high precision ($>80\%$) but max out at \textbf{41.77\%} EM, indicating partial-coverage behavior. 
\textit{Choice Funnel} narrows this gap on smaller open models; e.g., \textit{phi3-small} with \textit{Choice Funnel} exceeds the EM of larger models (e.g., Llama-90B, Mistral-Large V2) reported in Table~\ref{tbl:model_results_no_f1}.

\subsection{Bias Mitigation Analysis}
\label{subsec:bias_mitigation}
Section~\ref{sec:challenge} showed systematic \emph{under-selection} (CtAcc $\le 48\%$; negative CtDif with $p=1.70\times 10^{-6}$) and nontrivial \emph{selection/unselection} skew (SPD $>$ random; $p=0.0467$). 
\textit{Choice Funnel} directly targets both:
(i) \textbf{selection skew} is reduced via token debiasing (plug-in PriDe), lowering SPD and RStd/RSD;
(ii) \textbf{count bias} is corrected via adaptive stopping (confidence floor + NOTA), raising CtAcc and recall without sacrificing precision.
Qualitative audits show typical corrections where baselines output too few labels (e.g., returning $\{$\emph{offensive, hate}$\}$ in toxicity) while \textit{Choice Funnel} recovers the full set including \emph{threat} and \emph{harassment}.

\subsection{Efficiency}
\label{subsec:efficiency}
\textbf{InfCost} counts model forward passes per question. 
Option-wise \textit{yes/no} scales with the number of options $K$, whereas \textit{Choice Funnel} scales with the number of accepted selections plus at most one stop step (Sec.~\ref{sec:choicefunnel}). 
Empirically, \textit{Choice Funnel} reduces compute by \textbf{64.48\%} vs.\ \textit{yes/no} (Table~\ref{tbl:choice_funnel_model_results}), matching the analysis that cost tracks the number of correct labels rather than $K$.

\subsection{Domain- and Family-Level Trends}
\label{subsec:domain_family}
As noted in Sec.~\ref{sec:challenge}, different model families perform best on different \method\ domains (e.g., O3 on News/Events, GPT-4.1 on reading comprehension, Claude 3.7 on toxicity/law), underscoring that SATA tasks are heterogeneous. 
\textit{Choice Funnel} improves EM across all seven open models considered, suggesting its gains are architecture-agnostic.

\subsection{Ablations and Sensitivity}
\label{subsec:ablations}
Ablations (Appendix~\ref{app:ablation_stopping_condition}, \ref{app:ablation_cf_components}) show both stopping conditions are needed: removing either \texttt{NOTA} or the confidence floor $\tau$ degrades EM and CtAcc and increases SPD. 
Introducing \texttt{NOTA} \emph{after} the first accepted selection stabilizes early stopping (Appendix~\ref{app:idk_vs_nota_1}). 
We also report sensitivity to $\tau$ and to the number of permutations used to estimate option-ID priors for PriDe (Appendix).

\subsection{Human Baseline}
\label{subsec:human_baseline}
For reference, Table~\ref{tbl:model_results_no_f1} includes a \emph{non-expert human} baseline on \method. 
Human performance provides a ceiling that remains above most models’ EM, quantifying remaining headroom even after decoding improvements.

\subsection{Evaluation Design Sanity Check}
\label{subsec:eval_design}
To ensure fair credit for uncertainty-aware outputs, the main text includes a concise comparison of benchmark scoring (Table~\ref{tab:benchmark_excerpt}); the full comparison appears in Appendix~\ref{tab:benchmark_comparison}. 
Consistent with recent observations that binary grading penalizes abstention and can incentivize hallucination \citep{kalai2025hallucination}, \method\ additionally reports Jaccard-based scores. 
We emphasize that these metrics are \emph{supporting} diagnostics—our primary contribution is the decoding algorithm \textit{Choice Funnel}.


==> 7_Conclusion/conclusion-new.tex <==
\section{Conclusion}
\label{sec:conclusion}

We studied why LLMs underperform on Select-All-That-Apply (SATA) questions and showed that errors arise from \emph{systematic} behaviors—selection skew over option IDs and pervasive underestimation of the number of correct answers. To address these failures, we introduced \textbf{Choice Funnel}, a lightweight decoding algorithm that couples token debiasing with adaptive stopping and an explicit abstention path (NOTA). Across seven open-source models, Choice Funnel improves exact match, Jaccard, and count accuracy over strong baselines while reducing inference cost, converting partial knowledge into more complete answer sets.

A second contribution is \textbf{\method}, a human-validated, multi-domain diagnostic benchmark for multi-answer reasoning. Beyond enabling thorough analysis of selection and count bias, \method\ reports IDK-aware, set-overlap metrics alongside exact match, aligning evaluation with trustworthy reasoning and complementing Choice Funnel’s abstention mechanism.

Our results suggest a practical recipe for multi-answer decoding: \emph{debias first, then decide how many}, and allow abstention when evidence is weak. While performance remains below human ceilings and our stopping rule is heuristic, the method is modular (plug-in debiasers, flexible stopping) and efficient (cost scales with the number of accepted labels rather than total options). We see promising next steps in learned stopping criteria, structure-aware selection (e.g., label dependencies and constraints), and extending evaluation beyond \method\ to broader multi-label and multimodal settings.


==> Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{What Choice Funnel Teaches Us About Multi-Answer Reasoning}
Section~\ref{sec:challenge} showed that LLM failures on SATA stem largely from \emph{systematic} prediction behavior (selection skew and count underestimation), not merely lack of knowledge. 
By explicitly correcting option-ID priors and making \emph{adaptive} decisions about how many labels to select, 
Choice Funnel (Sec.~\ref{sec:choicefunnel}) converts partial knowledge into fuller set recovery (Sec.~\ref{sec:results}). 
Two practical takeaways emerge: (i) \emph{debiasing first, then deciding the set size} is more reliable than global thresholds; 
(ii) \emph{abstention} (NOTA) is valuable as a decoding primitive for trustworthy outputs.

\subsection{Generalization Beyond SATA-BENCH}
Although \method\ is our primary testbed, the decoding pattern of \emph{debias $\rightarrow$ iterative select $\rightarrow$ 
abstention/stop} is not specific to our benchmark. 
It applies to other multi-label settings where LLMs generate label IDs or short strings, e.g., 
taxonomy tagging, content moderation with multiple harm categories, or weakly supervised label discovery. 
We expect the efficiency advantage to persist in regimes where the number of \emph{true} labels per instance is small relative to the candidate set size ($C^\star \ll K$).

\subsection{Limitations}
\label{subsec:limitations}
\begin{itemize}[leftmargin=*,nosep]
\item \textbf{Heuristic stopping.} We use a fixed confidence floor $\tau$ for simplicity. While ablations show robustness, learned or instance-adaptive thresholds could further stabilize stopping under distribution shift.
\item \textbf{Debiaser estimation.} PriDe-style prior estimates rely on permutations over a holdout; their fidelity may vary by domain and option formatting. Poor estimates can under- or over-correct selection skew.
\item \textbf{Short-form choices.} Our decoding operates over short option identifiers. Tasks requiring longer free-form spans may need span-level calibration or constrained decoding.
\item \textbf{Coverage still below human ceiling.} Even with Choice Funnel, EM remains below non-expert human performance on \method\ (Table~\ref{tbl:model_results_no_f1}), indicating substantial remaining headroom.
\end{itemize}

\subsection{Threats to Validity}
\label{subsec:threats}
\begin{itemize}[leftmargin=*,nosep]
\item \textbf{Prompt sensitivity and position effects.} Option order/format can influence first-token distributions. We mitigate with prior correction and report RStd/RSD/SPD, but residual effects may remain.
\item \textbf{Threshold tuning leakage.} For probability-based baselines, the JI-optimal threshold is tuned on a small holdout (100 items). We keep it fixed for test and report bootstrap CIs; future work could use nested resampling.
\item \textbf{Extractor fallback.} For models without token probabilities, JSONL extraction failures are rare ($<3\%$ overall) but nonzero; our automated+human fallback could introduce minor bias (Appendix~\ref{app:prompts}).
\end{itemize}

%\subsection{Ethical Considerations and Broader Impact}
%\label{subsec:broader_impact}
%SATA-style decisions appear in sensitive domains (e.g., moderation, biomedicine, legal). 
%\emph{Under-selection} can suppress protected or safety-relevant labels; \emph{over-selection} can inflate false positives. 
%By enabling abstention and partial-credit evaluation (Jaccard), our setup encourages uncertainty-aware behavior rather than bluffing. 
%Compute-wise, Choice Funnel reduces forward passes relative to option-wise yes/no prompting (Sec.~\ref{subsec:efficiency}), lowering cost and carbon footprint for the same task.

%\subsection{Future Directions}
%\label{subsec:future}
%\begin{itemize}[leftmargin=*,nosep]
%\item \textbf{Learned stopping and calibration.} Replace the fixed $\tau$ with a learned criterion (e.g., temperature-scaled or meta-learned thresholds) and instance-adaptive NOTA scheduling.
%\item \textbf{Structure-aware selection.} Incorporate label dependencies (mutual exclusivity, hierarchy) via constrained or energy-based decoding to further raise EM without sacrificing precision.
%\item \textbf{From decoding to training.} Use Choice Funnel outputs as pseudo-labels or curriculum to train smaller models toward multi-answer calibration.
%\item \textbf{Broader evaluations.} Apply the method beyond \method, including multi-label classification corpora and multimodal SATA tasks, to stress-test generality.
%\end{itemize}


==> impact.tex <==
\section*{Impact Statement}

The introduction of \method marks a crucial advancement in evaluating Large Language Models (LLMs) on ``Select All That Apply" (SATA) multiple-choice questions. By addressing a significant gap in existing benchmarks, which predominantly focus on single-answer multiple-choice tasks, \method challenges LLMs with real-world scenarios requiring multiple correct responses across domains such as reading comprehension, law, and biomedicine. This benchmark highlights the limitations of current LLMs, which struggle to accurately determine all valid answers, achieving a best-case exact match accuracy of only $41.8\%$.

\method’s impact extends beyond evaluation, as it reveals key biases in LLM decision-making, such as count bias and selection bias, which hinder performance on multi-answer tasks. To address these shortcomings, the development of the \textit{Choice Funnel} algorithm demonstrates a novel approach to systematically improving LLM selection accuracy, significantly enhancing model performance in SATA tasks.

While the current focus is on knowledge-intensive domains, the potential for expansion into additional fields such as mathematics, coding, and instruction following is vast. \method can also be extended to free-text tasks, where the set of correct responses is not explicitly provided, and to other modalities, such as voice and vision. This would further refine LLM capabilities in handling complex, multi-faceted decision-making tasks. By pushing the boundaries of LLM evaluation, \method lays the foundation for the next generation of AI systems capable of more nuanced, flexible reasoning in diverse real-world applications.


\section*{Limitations}

\textbf{Memorization.} While we believe most questions in \method have not been seen during pretraining, we cannot fully rule out the possibility that some LLMs may have been exposed, even partially, to the source datasets. We do not have access to the pretraining data of proprietary models and therefore cannot conclusively assess memorization.

\textbf{Domain Coverage.} \method spans six diverse domains, including reading comprehension, biomedicine, and law. However, the total number of domains remains limited compared to larger-scale benchmarks such as MMLU, indicating that further expansion is needed for broader generalization.

\textbf{Text Modality.} Our benchmark is text-only. Real-world tasks often require multimodal reasoning (e.g., interpreting charts, images, or audio), which \method does not evaluate. We also do not address other data modalities, such as structured tabular data or sensor data, which are common in practical applications.

\textbf{Label Correctness.} Although we perform rigorous human validation and evaluations, we acknowledge that human beings can make mistakes. Some domains, such as biomedicine and law, are inherently complex and may contain subtle ambiguities. Thus, we cannot guarantee perfect correctness of all labels despite triple human annotation and agreement filtering.

\textbf{Language Limitation.} \method includes only English-language questions. Evaluating multilingual capabilities or cross-lingual transfer remains a work for the future.



==> related-work.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Multi-answer (SATA) datasets and benchmarks}
Most LLM benchmarks and training pipelines emphasize single-answer MCQs, limiting evaluation of multi-answer reasoning.
Existing SATA-style resources either present \emph{very large} label spaces (30+ labels per instance)—e.g., RCV1, BibTeX, StackExchange, HDLTex \citep{lewis2004rcv1,katakis2008bibtex,charte2015stackex,kowsari2017hdltex,aly2019hierarchical}—which makes exhaustive option selection impractical for prompt-based LLMs, or target narrow skills such as emotion or music style classification \citep{demszky2020goemotions,zhao2019review}.
Many also appear primarily in bag-of-words form and assume supervised training \citep{Liu_2022}, making them ill-suited for \emph{decoding-time} evaluation of general-purpose LLMs.
To our knowledge, no prior LLM benchmark consists exclusively of SATA questions in natural language with controlled distractors and human validation; we therefore introduce \method\ as a \emph{diagnostic} platform rather than a leaderboard.

\subsection{Selection/count bias and decoding calibration}
A growing literature documents option-format and position sensitivity in LLM MCQ answering—often termed \emph{selection bias} \citep{zheng2024mcq,wei2024selectionbias}.
Calibration/debiasing methods adjust first-token probabilities to offset priors over option identifiers, including RStd/RSD-style measures and the PriDe approach \citep{croce2020robustbench,reif2024calibration,zheng2024largelanguagemodelsrobust}.
However, most analyses and methods target \emph{single-answer} MCQ.
In the SATA setting, we observe two distinct phenomena (Sec.~\ref{sec:challenge}): (i) \emph{selection skew/avoidance} over option IDs (including an \emph{unselection} tendency), and (ii) pervasive \emph{count underestimation}.
Common heuristics (global thresholds over first-token probabilities; option-wise yes/no prompting) either ignore label interactions or inflate inference cost.
Our contribution differs in proposing a decoding-time algorithm—\emph{Choice Funnel}—that combines token debiasing with \emph{adaptive} stopping and an explicit abstention option, directly targeting both selection skew and count bias while remaining computationally light (Sec.~\ref{sec:choicefunnel}).

\subsection{Evaluation design, abstention, and IDK credit}
Benchmark scoring can inadvertently penalize uncertainty and reward bluffing.
Recent analysis argues that binary, all-or-nothing grading disincentivizes abstention and can increase hallucination \citep{kalai2025hallucination}.
Motivated by survey methodology that endorses explicit “I don’t know”/NOTA responses \citep{schumanpresser1996,Eckman2024}, 
\method\ reports set-overlap metrics (e.g., Jaccard) alongside EM to grant partial credit to uncertainty-aware outputs, aligning evaluation with trustworthy reasoning while keeping exact-set recovery as the strict target.
This evaluation design complements \emph{Choice Funnel}: the algorithm introduces an abstention path (NOTA), and the benchmark does not unduly penalize its use when appropriate.

\paragraph{Positioning.}
Prior work primarily (i) documents MCQ selection bias and (ii) calibrates option priors in single-answer settings.
We contribute a decoding algorithm that jointly mitigates selection \emph{and} count bias for multi-answer reasoning, and introduce \method\ as a human-validated testbed that diagnoses these biases and evaluates such algorithms.

